Continual Vision-Language Representation Learning with Off-Diagonal Information

Large-scale multi-modal contrastive learning frameworks like CLIP typically require a large amount of image-text samples for training. However, these samples are always collected continuously in real scenarios. This paper discusses the feasibility of continual CLIP training using streaming data. Unlike continual learning based on self-supervised learning methods for pure images, which is empirically robust against catastrophic forgetting, CLIP's performance degeneration in the continual setting is significant and non-neglectable. By analyzing the changes in the model's representation space during continual CLIP training from a spatial geometry perspective, we explore and summarize these spatial variations as Spatial Disorder (SD), which can be divided into Intra-modal Rotation and Inter-modal Deviation. Moreover, we empirically and theoretically demonstrate how SD leads to a performance decline for CLIP on cross-modal retrieval tasks. To alleviate SD, we propose a new continual vision-language representation learning framework Mod-X: Maintain off-diagonal information-matriX. By selectively aligning the off-diagonal information distribution of contrastive matrices, the Mod-X improves the capability of the multi-modal model by maintaining the multi-modal representation space alignment on the old data domain during continuously fitting the new training data domain. Experiments on commonly used datasets with different scales and scopes have demonstrated the effectiveness of our method.

==> content/10_acknowledgment.tex <==
\section{Acknowledgments}
This work has been supported in part by the NSFC (No. 62272411), the Zhejiang NSF (LR21F020004), Ant Group and Alibaba-Zhejiang University Joint Research Institute of Frontier Technologies.

==> content/7_experiment.tex <==
\section{Experiments}
\label{experiments}
\subsection{Training Datasets}
In the experiments, we use three image-text datasets varying in scale and scope to simulate continual CLIP training.
\textbf{MS COCO Captions} \cite{lin2014microsoft}: MS COCO Captions (COCO) is a widely used image caption dataset. It contains 80K training images, 30K validation images, and 5K testing images (COCO(5K)). Each image has 5 human-evaluated captions.
\textbf{Flickr30K} \cite{young2014image}: Flickr30K(F30K) contains 30K training images and 1K test samples (Flickr30K(1K)) collected from Flickr, together with 5 reference sentences provided by human annotators. \textbf{SBU-1M} \cite{ordonez2011im2text}: The SBU-1M collects 1M images from Flickr with associated visually relevant captions which representing a wider variety of content styles. After downloading and preprocessing, we utilized about 0.8M image-text pairs in our experiments. 

\subsection{Experiments Setting}
We apply our Mod-X framework to two experiment settings to illustrate that Mod-X helps the model not only better fits the newly trained data domain but also maintains the multimodal cognitive ability of the old data domain during the continual large-scale training.
\textbf{Experiment A:} The Experiment A follows the setup of the exploratory experiments, pre-training the CLIP$_0$ model using the COCO dataset. And then splitting Flickr30K dataset randomly and evenly into five sub-datasets and sequentially training them to update CLIP$_0$ continually.
\textbf{Experiment B:} Unlike Experiment A, which looks like fine-tuning, we try to simulate continual large-scale training in Experiment B. We train a CLIP from scratch using the joint data of COCO and Flickr30K (COCO+F30K) as the initial model CLIP$_0$ and continually train eight sub-datasets divided from the SBU-1M dataset, randomly and uniformly. Each sub-dataset contains 100K unique samples, an equal scale to the initial pre-training dataset (COCO+F30K). This experiment verifies that our framework can iterate under continual large-scale training and maintain or even improve the model’s cognition of past entities.
\textbf{Evaluation Details:} We use the test sets COCO(5K) and Flickr30K(1K) to evaluate the performance of model in continual training. And all the results in the tables and figures are the average of 3 runs with different seeds. Experiment details have been shown in Appendix \ref{Experiment_Setting}.

\iffalse
\subsection{Experiments Details}
\textbf{Training Details} We use ResNet50 \cite{he2016deep} as the vision encoder in CLIP, while the language encoder is a transformer-based architecture which follows modification proposed in CLIP \cite{OpenAi}. The input images are resized to 224 × 224 and the input texts are tokenized by WordPiece with a maximum length of 77. We utilize AdamW \cite{loshchilov2017decoupled} optimizer and a cosine annealing learning rate schedule with warmup which is consistent with \cite{OpenAi}. All of the experiments are conducted on 8 NVIDIA V100 GPUS. Details regarding hyper-parameter values for different experiments are provided in the Appendix \nzx{cite}.

\textbf{Evaluation Details.} We use the test sets of COCO(5K) and Flickr30K to evaluate the zero-shot image-text retrieval performance of CLIP model. 
\fi


\subsection{Performance of Mod-X in the Experiment A}
\label{experiment_A}
\iffalse
In figure \ref{fig:modx_f30k} , we show the effect of our framework Mod-X with (CLIP$_{Mod-X}$) or without (CLIP$_{w/o}$) Screening in continual CLIP training in Experiment A.
\begin{figure}[!h]
    \centering
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_i2t_coco.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_t2i_coco.pdf}
	%\label{fig:tsne-c4il}
	}
	
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_i2t_f30k.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_t2i_f30k.pdf}
	%\label{fig:tsne-c4il}
	}
	\caption{\nzx{need caption}
	}
	\label{fig:modx_f30k}
\end{figure}

From the results of zero-shot retrieval at each training phase, we can find that our framework, Mod-X, still has a good performance to the past pre-training dataset COCO during the continual training on the Flickr30K dataset. At each training phases, the zero-shot results of CLIP$_{Mod-X}$ on COCO(5K) testset does not show a significant drop, and the gap with the initial accuracy remained at $\pm 1$. In addition to this, by comparing the zero-shot retriveal results of the CLIP$_{cl}$ and CLIP$_{Mod-X}$ on the current training data domain (Flickr30K), it can be found that the CLIP$_{Mod-X}$ using the off-diagonal information before and after the model update is also significantly better than CLIP$_{cl}$ in continual fitting the current data domain. 
\fi

The Experiment A focuses on verifying that Mod-X can not only fit new data domains but also maintain a cognition of past data domains. This table shows the final multimodal retrieval performance of the different training strategies on COCO(5K) and Flickr30K(1K). The CLIP$_0$ is the initial pre-trained model based on the COCO dataset. The CLIP$_{ct}$ means training CLIP continually without any other operation. The CLIP$_{EWC}$ means using the EWC method \cite{kirkpatrick2017overcoming}, which is a typical regularization strategy in continual supervised learning. The CLIP$_{Mod-X}$ is the proposed Mod-X, and the CLIP$_{JT}$ is the joint training model using the joint datasets (COCO+F30K), which is an upper bound for continual CLIP training in Experiment A. The detailed performance of the different models at each training phase is shown in Appendix \ref{detailed_A}.

\begin{table*}[!h]
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
& & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
& & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
\multirow{4}{*}{COCO} & CLIP$_{0}$ & \overline{16.9} & 37.0 & 46.2 & \overline{14.7} & 34.2 & 47.0 & \overline{12.0} & 30.0 & 41.0 & \overline{10.6} & 29.6 & 41.0  \\
 & CLIP$_{ct}$ & 20.6 & 42.8 & 56.4 & 6.2 & 17.8 & 26.1 & 16.1 & 38.5 & 50.4 & 4.7 & 14.3 & 21.8 \\
 & CLIP$_{EWC}$ & 22.2 & 43.1 & 57.0 & 6.1 & 17.2 & 26.5 & 17.0 & 39.1 & 51.2 & 4.5 & 13.9 & 22.0 \\
 %& CLIP$_{w/o}$ & 24.9 & 50.4 & 60.3 & 7.6 & 21.4 & 30.9 & 19.4 & 43.2 & 54.6 & 6.0 & 17.4 & 25.7 \\
 & CLIP$_{Mod-X}$ & \textbf{27.9} & \textbf{53.4} & \textbf{64.4} & \textbf{14.5} & \textbf{34.0} & \textbf{46.1} & \textbf{20.2} & \textbf{45.0} & \textbf{57.2} & \textbf{10.1} & \textbf{26.4} & \textbf{37.4} \\
\midrule
COCO+F30K & CLIP$_{jt}$ & \underline{30.1} & 55.9 & 60.1 & \underline{16.1} & 38.1 & 51.9 & \underline{22.5} & 48.5 & 59.6 & \underline{11.7} & 30.9 & 42.7 \\ %
\bottomrule
\end{tabular}
\caption{The final multimodal retrieval performance of the different continual CLIP training strategies in the Experiment A.}
\label{table:modx_f30k}
\end{center}
\vspace{-0.5em}
\end{table*}
%The underlined values represent the upper bound for continual training of the CLIP. And the bold ones are the results of our framework Mod-X. 
From the results in the Table \ref{table:modx_f30k}, it is clear that our method CLIP$_{Mod-X}$
%it can be found that the final performance of our method far exceeds the results of CLIP$_{cl}$.
maintains its multimodal retrieval results on COCO(5K) after completing continual training on Flickr30K. The gap between CLIP$_0$ and CLIP$_{Mod-X}$ is just 0.2\% points in image-text retrieval and 0.5\% points in text-image retrieval on COCO(5K). At the same time, the retrieval results of the CLIP$_{Mod-X}$ on the test set Flickr30K(1K) are also affected by the training domain and have a significant increase. The $R@1$ performance of the CLIP$_{Mod-X}$ in image-text retrieval rise from 16.9\% (in CLIP$_0$) to 27.9\%. And the $R@1$ results in text-image retrieval increase from 12.0\% (in CLIP$_0$) to 20.2\%. The performance gap between CLIP$_{Mod-X}$ and CLIP$_{jt}$ on the Flickr30K is only at most 2.3\% points. Conversely, due to the model's cognitive disorder in continual training, the performance of CLIP$_{ct}$ on COCO(5K) drops significantly. In addition, although the performance of CLIP$_{ct}$ on Flickr30K(1K) has improved, it is still far from the upper bound CLIP$_{jt}$. The EWC, as a typical regularization strategy in continual learning, selectively updates the model by evaluating the importance of each parameter of the model. From the above experimental results, although CLIP$_{EWC}$ improves the accuracy of continual CLIP training on Flickr30K(1K), it does not preserve the model's understanding in past samples (COCO(5K)). According to the above comparisons, we can conclude that our Mod-X framework can not only maintain the cognitive ability on past samples during continual CLIP learning but also improve the model's fitting ability to the current training data domain.


%outperforms CLIP$_{cl}$ 7.3 and 8.3 points on Image-Text retrieval results. In the Text-Image retrieval results, it also exceeds 4.1 and 5.4 points. Compared with the upper bound CLIP$_{JT}$, the gap is only 2.3 points at most (the R@1 result in Text-Image Retrival on Flickr30K). The low performance of traditional regularization methods EWC also shows that multi-modal continual training is more complex than single-modal supervised training. 

%Beside this, we compare the performance of Mod-X with CLIP$_{Mod-X}$ and without CLIP$_{w/o}$ Screening during continual training in Experiment A. We can see that the multimodal retrieval performance of Mod-X without the Screening CLIP$_{w/o}$ in the COCO data domain is only 1 point higher than that of CLIP$_{cl}$, and the gap with CLIP$_{Mod-X}$ is obvious. Moreover, the results of CLIP$_{w/o}$ is also lower than CLIP$_{Mod-X}$ on the current Flickr30K data damain (3 points in image-text $R@1$ and 0.8 points in text-image $R@1$ on Flickr30K). All of this shows that Screening plays an important role in Mod-X. Aligning this misunderstanding of the old model with the concept of new objects will affect the parameter update of the entire CLIP model in the continual training. 

%从每个阶段zero-shot retrieval的结果中我们可以看出我们的新框架ModX在F30K数据集上进行连续更新的过程中其对过去的预训练数据集COCO的拟合能力依旧很好。其zero-shot retrieval的表现没有出现明显的下降（正负1）。这说明我们的方法的确帮助模型缓解了对过去样本的概念模糊。除此以往，通过比较模型在当前训练数据集（Flickr30K）上的zero-shot retriveal表现可以发现，我们的方法在拟合当前数据时由于对非对角线信息的保存，使得最终的拟合效果也明显优于continual training。下表展示了CLIP_Mod-X模型在连续更新之后的最终表现。
\iffalse
\subsection{The importance of Screening}
To illustrate the importance of Screening, we compare the performance of Mod-X with and without Screening during continual training in Experiment A. The results of CLIP$_{w/o}$ can be seen in figure \ref{table:modx_f30k}. We can see that the zero-shot retrieval performance of Mod-X without the Screening CLIP$_{w/o}$ drops significantly. At the same time, the performance of the CLIP$_{w/o}$ in the current data domain (Flisckr30K) also fluctuates significantly during the continual training compared to CLIP$_{Mod-X}$. Comparing the final retrieval results of the three training strategies in Table \ref{table:modx_f30k}, it can be find that the performance of the CLIP without Screening CLIP$_{w/o}$ in the past data domain is only 1 point higher than that of CLIP$_{cl}$, and the gap with CLIP$_{Mod-X}$ is obvious. Moreover, the results of CLIP$_{w/o}$ is also lower than CLIP$_{Mod-X}$ on the current data damain (3 points in image-text $R@1$ and 0.8 points in text-image $R@1$ on Flickr30K). All of this shows that Screening plays an important role in Mod-X. Aligning this misunderstanding of the old model with the concept of new objects can affect the parameter update of the entire model in the continual training.
\fi

\subsection{Performance of Mod-X in the Experiment B}
\label{experiment_B}
%In the Experiments B,  we use SBU1M dataset to simulate large-scale continual CLIP training. The difference from the Experiment A is that we use COCO+F30K as the pre-training data for the initial pre-trained model CLIP$_0$. Joint Datasets are the union of COCO, F30K and SBU1M. And the number of training phases increased from 5 to 8. The amount of training data in each training phase reaches 100K which is approximately equal with pre-trained datasets COCO and F30K.
Unlike Experiment A, which looks like fine-tuning, Experiment B focuses on verifying that our framework Mod-X can maintain or even improve the model’s understanding of past entities when iterating under continual large-scale training. Table \ref{table:modx_sbu1m} shows the final multimodal retrieval performance of the different continual CLIP training strategies in Experiment B. The detailed $R@1$ results in each training phase can be seen in Appendix \ref{detailed_B}.

\begin{table*}[!h]
\vspace{-0.5em}
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
& & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
& & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
\multirow{4}{*}{COCO+F30K} & CLIP$_{0}$ & \overline{33.0} & 56.5 & 67.3 & \overline{17.7} & 40.7 & 52.9 & \overline{23.4} & 48.2 & 59.1 & \overline{12.9} & 32.8 & 44.9  \\
 & CLIP$_{ct}$ & 5.4 & 16.0 & 23.3 & 3.0 & 9.0 & 14.0 & 3.6 & 12.0 & 18.6 & 2.3 & 7.3 & 11.4 \\
 & CLIP$_{EWC}$ & 6.1 & 18.2 & 33.5 & 3.1 & 11.7 & 18.2 & 3.3 & 10.4 & 16.2 & 2.1 & 5.4 & 10.0 \\
 %& CLIP$_{w/o}$ & 24.9 & 50.4 & 60.3 & 7.6 & 21.4 & 30.9 & 19.4 & 43.2 & 54.6 & 6.0 & 17.4 & 25.7 \\
 & CLIP$_{Mod-X}$ & \textbf{37.3} & \textbf{62.6} & \textbf{72.1} & \textbf{19.5} & \textbf{42.8} & \textbf{55.7} & \textbf{26.0} & \textbf{51.9} & \textbf{62.6} & \textbf{13.4} & \textbf{33.6} & \textbf{45.3} \\
\midrule
Joint Datasets & CLIP$_{jt}$ & \underline{39.3} & 71.5 & 81.1 & \underline{25.1} & 51.6 & 64.3 & \underline{27.8} & 54.9 & 66.5 & \underline{15.9} & 38.6 & 51.3 \\ %
\bottomrule
\end{tabular}
\caption{The final multimoal retrieval performance of the different continual CLIP training strategies in the Experiment B.}
\label{table:modx_sbu1m}
\end{center}
\vspace{-0.5em}
\end{table*}

Compared to the initial pre-trained model CLIP$_0$, our CLIP$_{Mod-X}$ not only does not show a significantly drop such as CLIP$_{ct}$ in multimodal retrieval performance on COCO(5K) and Flickr30K(1K) but it also shows a slight improvement after continual training in SBU-1M. The image-text $R@1$ results on Flickr30K(1K) increase from 33.0\% to 37.3\% and the accuracy on COCO improved to 19.5\% from 17.7\%. The performance of text-image $R@1$ is the same as that of image-text. The accuracy increase from 23.4\% to 26.0\% on Flickr30K(1K) and 12.9\% to 13.4\% on COCO(5K). The gap between continual CLIP training and joint training has been somewhat narrowed. Conversely, the ability of cognitive alignment in CLIP$_{ct}$ and CLIP$_{EWC}$ are lost in the large-scale data. This results in verifying that our framework Mod-X can iterate under continual large-scale training and can maintain or even improve the model’s cognitive ability of past entity concepts.






==> icml2023_hawaii_camera_ready__1_/content/10_acknowledgment.tex <==
\section{Acknowledgments}
This work has been supported in part by the NSFC (No. 62272411), the Zhejiang NSF (LR21F020004), Ant Group and Alibaba-Zhejiang University Joint Research Institute of Frontier Technologies.

==> icml2023_hawaii_camera_ready__1_/content/1_abs.tex <==
\begin{abstract}
%Multi-modal pre-trained methods with a contrastive learning framework (like CLIP) require a large amount of image-text samples for training. 
Large-scale multi-modal contrastive learning frameworks like CLIP typically require a large amount of image-text samples for training. However, these samples are always collected continuously in real scenarios. This paper discusses the feasibility of continual CLIP training using streaming data. Unlike continual learning based on self-supervised learning methods for pure images, which is empirically robust against catastrophic forgetting, CLIP’s performance degeneration in the continual setting is significant and non-neglectable.
%Unlike continual learning based on self-supervised learning methods for pure images, the performance of CLIP on cross-modal retrieval tasks is significantly lower in a continual training setting than joint training setting. 
By analyzing the changes in the model's representation space during continual CLIP training from a spatial geometry perspective, we explore and summarize these spatial variations as \textbf{Spatial Disorder (SD)}, which can be divided into \textbf{Intra-modal Rotation} and \textbf{Inter-modal Deviation}. 
%Intra-modal Rotation means that the vision and language representation space in the continual CLIP training is rotating greatly around the center of a high-dimensional unit sphere, accompanied by a relatively small change in the topology of the representation space. Inter-modal deviation happens when the vision and language's intra-modal rotation is unsynchronized.
Moreover, we empirically and theoretically demonstrate how SD leads to a performance decline for CLIP on cross-modal retrieval tasks. To alleviate SD, we propose a new continual vision-language representation learning framework \textbf{Mod-X}: \textbf{M}aintain \textbf{o}ff-\textbf{d}iagonal information-matri\textbf{X}. By selectively aligning the off-diagonal information distribution of contrastive matrices, the Mod-X improves the capability of the multi-modal model by maintaining the multi-modal representation space alignment on the old data domain during continuously fitting the new training data domain. Experiments on commonly used datasets with different scales and scopes have demonstrated the effectiveness of our method.


%Multimodal pre-trained methods with a contrastive learning framework (like CLIP) have recently achieved consistent advantages on various cross-model downstream tasks. However, they usually require a vast computing budget and a large amount of image-text samples for training, while this samples always is collected continuously in real scenarios. In this paper, we discuss the feasibility of continual training CLIP model based on discrete streaming data. We find that the multimodal retrieval performance of the CLIP in a continual training setting is significantly lower than that in a joint training setting, which is clearly different from single-image self-supervised continual training. We name this phenomenon \textbf{Spatial Disorder(SD)}. By tracking the changes of the representation vectors in the continuously updated CLIP model, we explore and summarize the variation of the modal encoders within the CLIP: \textbf{Intra-modal Rotation} and \textbf{Inter-modal Deviation}. Intra-modal Rotation means that the vision and language representation space in the continual CLIP training is rotating greatly around the center of a high-dimensional unit sphere, accompanied by a relatively small change in the topology of the representation space. Inter-modal deviation happens when the vision and language's intra-modal rotation is unsynchronized. Moreover, we empirically and theoretically demonstrate how intra-modal rotation and inter-modal deviation lead to a decline in CLIP's retrieval performance. In order to alleviate spatial disorder in continual CLIP training, we propose a new continual vision-language representation learning framework \textbf{Mod-X}: \textbf{M}aintain \textbf{o}ff-\textbf{d}iagonal information-matri\textbf{X}. By selectively aligning the off-diagonal information distribution of contrastive matrixes, the Mod-X helps the model not only better fits the newly trained data domain but also maintains the multimodal representation alignment on the old data domain during the continual training (Section \ref{experiments}).

%Contrastive cross-modal pre-trained models CLIP get a consistent performance in downstream tasks. However, since training such a model requires millions of image-text samples and a lot of computing resources, retraining is expensive and not easy to modify when biases or errors occur in the model. In this paper, we discuss the feasibility of training CLIP models based on discrete streaming data continuously. We find that the multi-modal retrieval results of CLIP in continual training are significantly lower than joint training. We name this phenomenon \textbf{Concept Indistinct (CI)}. By analyzing the representation space variation of the modal encoders within the CLIP during continual training, we find that the reason for the concept indistinct in continual CLIP training comes from the \textbf{Intra-modal Rotation} and \textbf{Inter-modal Deviation}. Moreover, we mathematically give the conditions under which the inter-modal deviation leads to concept indistinct during continual CLIP training. To this end, we propose a new continual training framework \textbf{Mod-X}: \textbf{M}aintain \textbf{o}ff-\textbf{d}iagonal information-matri\textbf{X}. By selectively aligning the off-diagonal information distribution of the contrastive matrix, the Mod-X not only better fits the newly trained data domain, but also maintains the multimodal concept alignment of the old data domain during the continual CLIP training. 

%基于对比的多模态预训练模型CLIP在下游任务中获得了优良的表现。然而，获得这样一个预训练模型需要百万级别的图片文字对和大量的计算资源。在这篇论文里，我们讨论基于离散的数据流连续训练clip模型的可行性。我们发现单纯的连续训练CLIP模型会使得模型的表征泛化能力明显低于全量数据下的训练，我们将这样的现象命名为表征的灾难性遗忘。同时我们发现导致表征泛化性下降的原因来自模型离散训练阶段模态内旋转和模态间偏移。为此，我们提出了一种基于对比的连续多模态训练策略---XXXX，通过合理蒸馏对比矩阵中非对角线分布信息，使得XXX模型在连续训练过程中保留模型对之前数据的泛化能力同时还能拟合新训练的数据。

\end{abstract}

==> icml2023_hawaii_camera_ready__1_/content/2_intro.tex <==
\section{Introduction}
Recently, multi-modal pre-trained models such as CLIP \cite{radford2021learning} have attracted much attention. By utilizing these pre-trained models, many works have achieved new progress in downstream tasks such as image classification, semantic segmentation, object detection, speech recognition \cite{wei2022mvp,wang2021dense,xie2021detco,baevski2020wav2vec}, etc. Although the CLIP model has strong generalization in open-world data, as mentioned in its original paper \cite{radford2021learning}, the ability to match image-text samples that are not in its training data distribution is still weak. The natural idea to alleviate this problem is to scale up the training data that covers different data domains. However, it is impractical to train infinite data distribution with limited hardware resources at once. %And due to the high training cost, it is impractical to retrain it when biases or errors are found in such a large-scale vision-language model. %it becomes extremely difficult to modify the pre-trained model itself when biases or errors are discovered in model's representation.
\iffalse
\begin{figure}[b]
\vspace{-1em}
	\centering
	\includegraphics[height=0.9in]{./figure/process}
	\caption{The Schematic diagram of continual CLIP training and joint training. Different colors in the sub-dataset represent different subsets split from the joint-dataset.}
	\label{Schematic_diagram}
\vspace{-1em}
\end{figure}
\fi

To address the above problems, this paper mainly explores the feasibility of continuously training the CLIP model through streaming data, a training paradigm that follows Continual Learning (CL) \cite{mccloskey1989catastrophic}. Traditional supervised continual learning has been proven to suffer from catastrophic forgetting \cite{rebuffi2017icarl,kirkpatrick2017overcoming}: The model's performance on old tasks drops significantly as training phases rising. Recently, some works \cite{ni2021self,hu2021well} have validated that self-supervised models based on pure images like SimCLR \cite{chen2020simple} and BarlowTwins \cite{zbontar2021barlow} do not suffer from severe catastrophic forgetting during continual training. Some works \cite{madaan2021representational,thai2021does} conjecture that the reason is that the contrastive loss is not directly affected by the supervised signal, and the self-supervised framework does not have a Softmax function to amplify the influence of labels.%difference between the samples based on their label. % and the contrastive loss is not affected by the supervised signal. %Based on these two points, the self-supervised model avoids the occurrence of catastrophic forgetting in the CL.

%To simulate continual CLIP training, we randomly and evenly divide the training data (joint-dataset) into multiple sub-datasets and train the CLIP sequentially using these sub-datasets. For comparison with continual training, we train a CLIP additionally from scratch using the joint-dataset, which is named joint training, as the upper bound on the performance of the continuously trained model. 
\iffalse
The entire continual training process is shown in Figure \ref{Schematic_diagram}. 

\begin{figure}[t]
	\centering
	\includegraphics[height=0.9in]{./figure/process}
	\caption{The Schematic diagram of continual CLIP training and joint training. Different colors in the sub-dataset represent different subsets split from the joint-dataset.}
	\label{Schematic_diagram}
	\vspace{-1em}
\end{figure}
\fi

%To simulate continual CLIP training, we randomly and evenly divide the training data (joint-dataset) into multiple sub-datasets and train the CLIP sequentially using these sub-datasets. For comparison with continual training, we train a CLIP additionally from scratch using the joint-dataset, which is named joint training, as the upper bound on the performance of the continuously trained model. 

However, the performance of CLIP with a continual training setting is clearly different from the self-supervised continual training, which only uses images, though they both utilize contrastive loss. There is a significant degradation of multi-modal retrieval results with continual CLIP training compared with joint training (the experiment results are shown in Section \ref{explore} and \ref{experiments}). 
%The performance of CLIP in  image-text retrieval decreased significantly during continual CLIP training. 
By analyzing the changes in the model's representation space during continual CLIP training from a spatial geometry perspective,
%By analyzing the representation space changes of CLIP model from a spatial geometry perspective, 
%Due to the vision and language encoders within the CLIP normalizing the representation to a unit vector through a dimension-based $L_2$ norm, which limits the diffusion of representation vectors length, we try to analyze the representation space variation of modal extractors from a spatial geometry perspective. By tracking the directional changes of the representation vectors in the continuously updated CLIP model (in Section \ref{explore}), 
we explore and summarize these spatial variations as \textbf{Spatial Disorder (SD)}, which can be divided into \textbf{Intra-modal Rotation} and \textbf{Inter-modal Deviation}. The intra-modal rotation represents the representation space of the single-modal feature extractor (vision or language) within the CLIP rotates around the center of the high-dimensional sphere.
%, accompanied by a slow topology change during the continual CLIP training. 
The inter-modal deviation represents the shift of representation alignment of different modal extractors (vision and language) to the same entities during continual training. Moreover, we demonstrate how intra-modal rotation and inter-modal deviation lead to a performance decline for CLIP on cross-modal retrieval tasks in both empirically and theoretically.
%(in Section \ref{explore}).

%What’s more, we demonstrate mathematically that inter-modal deviation leads to concept indistinct (in Section \ref{explore}).  
%Beside this, we also give the conditions under which the inter-modal deviation leads to concept indistinct from the perspective of mathematics.
To alleviate this SD in continual CLIP training, we %introduce the distillation strategy from traditional continual learning and 
propose a simple yet effective framework Mod-X: \textbf{M}aintain \textbf{o}ff-\textbf{d}iagonal information-matri\textbf{X}. Unlike contrastive loss \cite{oord2018representation} only focuses on widening the similarity gap between positive and negative sample pairs, the Mod-X framework pays more attention to representation space alignment. The elements in the contrastive matrix represent the similarity between visual and textual entities, which also refer to the included angle between visual and textual representation vectors when the length of vectors is \textbf{1}. The angle distribution between the vectors represents the inherent representation space structure of the model under the current samples. 
%Different representation vectors, activated by samples, represent different regions of the model's representation space. Therefore, the contrastive matrix constructed by the model based on samples not only shows the similarity between visual and textual entities, but also shows the partial representation space distribution of the model.
%The elements in the contrastive matrix represent the similarity between visual and textual entities, which also refer to the included angle between visual and textual representation vectors. Because of this, the elements distribution in the contrastive matrix is equivalent to the structure of the representation space of the model. 
By selectively aligning the distribution of the off-diagonal elements, Mod-X preserves the spatial relationships between modals of various old entities while fitting the current vision-language data during continual training.
%\nzx{Each element in the contrastive matrix represents the similarity or spatial relationships between visual and textual entities. By selectively aligning the off-diagonal information distribution constructed by the current and past models based on the recent training samples, Mod-X preserves the correct correspondence between modals of various old entities while fitting the current vision-language data during continual training.} 
The experiments (in Section \ref{method}, \ref{experiments} and Appendix \ref{Appendix_to_experiments}) on commonly used datasets with different scales and scopes show that our Mod-X framework improves the capability of the multi-modal model by maintaining the multi-modal representation space alignment on the old data domain during continuously fitting the new training data domain. %More experiment details have been shown in Appendix \ref{Appendix_to_experiments}.
%From the results in Experiment A, we can find that Mod-X effectively reduces the concept indistinct of the CLIP model during continual training on Flickr30K dataset. It's multimodal retrieval performance on the COCO(5K) dataset remains the same as the initial accuracy. What's more, its performance on the test set of Flickr30K continued to rise, and at the end of the continual training, Mod-X's performance on the Flickr30k test set was only 2 points worse than the upper bound of joint training. 
The contributions of this paper are summarized as follows:
\begin{itemize}
\item We discuss the feasibility of training the CLIP model continuously through streaming data. Empirical experiments demonstrate that continual CLIP training leads to persistent performance degrades on cross-modal retrieval tasks, which is  different from the phenomenon of continual learning based on self-supervised learning methods for pure images.

\item We explore and summarize the model's spatial variation during continual CLIP training as Spatial Disorder, which can be divided into intra-modal rotation and inter-modal deviation. Furthermore, we demonstrate how spatial disorder leads to a performance decline for CLIP on cross-modal retrieval tasks in both empirically
and theoretically (in Section \ref{explore}).

\item We propose a simple yet effective continual CLIP training framework \textbf{Mod-X} that alleviates space disorder during continual CLIP training by selectively aligning contrastive matrices' off-diagonal information. Experiments (in Section \ref{experiments} and Appendix \ref{Appendix_to_experiments}) on commonly used datasets with different scales and scopes have evaluated the effectiveness of our method.
\end{itemize}

%1.跨模态预训练模型CLIP的使用现状 2.缺点（为什么我们要做连续clip的原因） 3.我们做了连续clip之后发现了什么* 现象（模型表征泛化性下降） *原因（模态内旋转和模态间偏移）
%4.我们怎么改进，得到什么样的结果 
%5.贡献和缺陷


%目前越来越多的工作关注到了多模态预训练模型的优势，尤其是基于clip的自监督多模态预训练模型。由于其训练过程不需要标注信息，大大减少了模型训练的成本。同时由于其图片文字对数据的易获得性，也让clip可以在超大规模的open word 数据集上进行训练。通过利用这些预训练好的模型，许多工作在下游任务比如图片分类，语义分割，物体识别，语音识别等等方面取得了进一步的进展。然而，正如CLIP原文所说，虽然CLIP可以在大规模数据上进行训练，但其依旧会对不在其训练数据分布中的样本失去判断能力。并且由于其训练成本过高，当发现模型本身的偏置或者错误时，对其进行修改变得极其困难。因为重新训练一个模型需要大量的计算资源。同时，储存和获得大规模的数据本身所消耗的成本也极其巨大。

%因此，在这篇论文中，我们尝试探讨CLIP模型在离散数据集间连续训练的可行性。正如流程图1所示，我们将预训练的全数据集随机切分成数量相同的若干个子集，然后在多个子集上顺序训练CLIP模型。这样的训练方式不但可以

%通过对每个训练阶段模型表征质量的评估，我们发现与之前基于图片的单模态自监督连续学习给出的结论不同：连续自监督对比学习不会降低模型的泛化性能，在多模态下，模型表征的泛化性随着连续训练阶段的上升而明显下降。也即模型对图文的概念在连续训练过程变得模糊和不确定（概念模糊）。

%为了







==> icml2023_hawaii_camera_ready__1_/content/3_relate.tex <==
\section{Related Work}
\textbf{Continual Learning.} Continual learning (CL) \cite{thrun1995lifelong}, or incremental learning, mainly focuses on supervised tasks. In addition to the vision-based tasks \cite{de2021continual,kj2021incremental,cha2021ssul,ahn2021ss}, some works discuss language-based tasks \cite{biesialska2020continual,sun2019lamol}. We can summarize the existing continual learning methods into three categories: regularization \cite{kirkpatrick2017overcoming,ahn2019uncertainty,ni21revisit}, replay \cite{rebuffi2017icarl,rolnick2019experience,wang2021ordisco}, and architecture \cite{thai2021does,ni2021self,hu2021well,madaan2021representational}. However, traditional supervised continual learning methods are limited by labels and unsuitable for self-supervised or unsupervised situations.

\quad In unsupervised and self-supervised single-modal continual training, the latest work \cite{thai2021does,ni2021self,hu2021well,madaan2021representational} has drawn some conclusions different from those of supervised continual learning. However, only a few pieces \cite{srinivasan2022climb,fan2022unified} focus on incremental multi-modal learning. However, \cite{srinivasan2022climb} did not propose a new method to alleviate the catastrophic forgetting problem in multimodal continual learning. Instead, it provided baselines for the state-of-the-art supervised unimodal continual learning methods when applied to some single-model multimodal tasks. And \cite{fan2022unified} discussed continuous updates in multimodal graphs, which is far from our intended goal of continuously updating multimodal pre-trained models. Because of the cooperation between different modalities, continual multi-modal pre-training shows different performance and complex problems from single-modal continual training.

%We can summarize the existing continual learning methods into three categories: regularization, replay and architectural. The regularization approaches \cite{kirkpatrick2017overcoming,ahn2019uncertainty,ni21revisit} guides current model updates by introducing regularization constraint. Replay-based CL methods \cite{rebuffi2017icarl,rolnick2019experience,wang2021ordisco} store some previous data and replay them into current training. And the architectural strategies \cite{li2019learn,araujo2022entropy} set specific model parameters or add model structures for each task. In the field of unsupervised and self-supervised based on single modal, the latest work \cite{thai2021does,ni2021self,hu2021well,madaan2021representational} has drawn some conclusions different from those of supervised. However, only a few works \cite{srinivasan2022climb,fan2022unified} focus on incremental multimodal tasks learning. Because of the mutual cooperation between different modals, continual multimodal pre-training shows different performance and problems from single modal continual training.


\textbf{Visual-Language Representational Learning.} Vision-language representation learning based on contrastive loss \cite{oord2018representation}, such as CLIP \cite{radford2021learning}, has attracted a lot of attention in various fields \cite{radford2021learning,li2021supervision,andonian2022robust}. And the pre-trained model performs surprisingly well on downstream tasks \cite{shu2022test,wang2022learning,chowdhury2022novelty}. At the same time, the large-scale image-text datasets, e.g., Laion400M \cite{schuhmann2021laion} and Conceptual Captions \cite{sharma2018conceptual}, have played a key role in multimodal pre-training. Although large-scale open-world datasets contain various samples, the pre-trained model still loses the ability to perfectly match image-text sample pairs that are not in its training data domain \cite{radford2021learning}. 

%The natural idea to alleviate this problem is to scale up the training data to cover different data domains. However, it is infeasible to train infinite data with limited hardware at once. Therefor, we explore the feasibility of training CLIP model continuously through streaming data and propose a new framework Mod-X to alleviating CLIP's Concept Indistinc (CI).

%And due to its expensive cost in training, when biases or errors are discovered in such a large-scale vision-language model, retraining it using other datasets is impractical. Because of this, we explore the feasibility of training CLIP model continuously through streaming data and propose a new framework Mod-X to alleviating CLIP's Concept Indistinc (CI).

%现阶段的连续学习主要集中在有监督任务，除了基于图片的任务以外也出现了一些讨论语言模型的工作。他们缓解灾难性遗忘的方法主要可以分为三种形式。分别为正则化 回溯 以及结构化策略。在基于单模态的无监督和自监督领域，最新的工作则得出了一些与有监督不一样的结论。然而这些工作并没有关注到多模态的预训练。由于模态间的相互合作，连续多模态预训练表现出了和单模态自监督不一样的结果和原因。

%基于对比误差的vision-language表征学习得到了越来越多的关注。通过对比框架measuring the similarities of positive and negative pairs have gained a lot of attention in the com- munity. 同时现有的大规模数据集也扮演了很重要的角色。通过大规模数据得到的预训练模型在下游任务中获得了令人惊喜的表现。然而数据是实时，使用有限的计算资源来训练无限的数据是不切实际的。为此，“然而预训练模型依旧会受到训练数据域的影响，同时”







==> icml2023_hawaii_camera_ready__1_/content/4_explori.tex <==
\begin{figure*}[t]
%\vspace{-0.5em}
    \centering
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/base_I2T_COCO.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/base_T2I_COCO.pdf}
	%\label{fig:tsne-c4il}
	}
    \vspace{-.5em}
	
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/base_I2T_f30k.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/base_T2I_f30k.pdf}
	%\label{fig:tsne-c4il}
	}
	\vspace{-1em}
	\caption{The multi-modal retrieval $R@1$ results of CLIP$_t$ $(0\leq t\leq 5)$ on test sets COCO (5K) and Flickr30k (1K). The two sub-figures on the left show the Image-Text retrieval $R@1$ performance of CLIP$_t$ on the continual training phase $t$. The initial training phase represents the performance of CLIP$_{0}$. The rights show the Text-Image $R@1$ results of CLIP$_t$ on the continual training phase $t$. The pentagon points (CLIP$_{jt}$) show the results of the CLIP under joint training, which is an upper bound for continual CLIP training (CLIP$_{ct}$).
	}
	\vspace{-.5em}
	\label{fig:base_retrival}
\end{figure*}
\section{Spatial Disorder in Continual CLIP}
\label{explore}
%在这一节，我们详尽讨论了预训练CLIP模型在连续训练过程中其模型的zero-shot图文检索能力的表现。并将模型表现能力的下降命名为概念模糊。同时发现了导致模型出现概念模糊的原因：1.2。最后我们以数学证明的方式给出了CLIP模型在连续学习过程中出现模态间旋转的可能性。
%1.实验设置
%2.评估方式
%3.实验现象
%4.原因
%5.证明
%6.
This section mainly aims to explore the characteristics of the CLIP model while training continually. By analyzing the changes in the model’s representation space from a spatial geometry perspective during continual CLIP training, we explore and summarize these spatial variations as Spatial Disorder (SD), which can be divided into intra-modal rotation and inter-modal deviation. Then, we demonstrate how intra-modal rotation and inter-modal deviation lead to a performance decline for CLIP on cross-modal retrieval tasks in both empirically and theoretically, respectively.

\textbf{Exploration Setup.} 
To ensure the controllability of the exploration, we train a CLIP$_0$ model from scratch on the COCO dataset \cite{lin2014microsoft} based on the OpenAI source code \cite{OpenAi} and use it as the initial state (start) of continual CLIP training. After that, we divide the Flickr30K dataset \cite{young2014image} into five sub-datasets \{$D_1$,$D_2$,$D_3$,$D_4$,$D_5$\} uniformly and randomly to simulate streaming data. Then we train the CLIP$_0$ based on these sub-datasets sequentially. We name this pure continual training without other operations as CLIP$_{ct}$.
%, and no other data is used when training on each sub-dataset. 
After finishing five training phases, we obtain the model CLIP$_5$. For comparison with CLIP$_{5}$, we joint training a CLIP$_{jt}$ model using joint dataset COCO and Flickr30K, as the upper bound of the CLIP$_{5}$. The hyper-parameters for all training phases are kept the same, and detailed settings of CLIP model and training hyper-parameters can be seen in Appendix \ref{Experiment_Setting}. 

%The vision encoder in CLIP$_0$ is RN50 \cite{he2016deep} and language encoder is a transformer-based architecture which follows modification proposed in CLIP \cite{OpenAi}. In the first training phase, we inherit the parameters of CLIP$_0$ and train it on subset $D_1$ to obtain model CLIP$_1$. Then train the CLIP$_1$ on subset $D_2$ and no other data is used when training on each sub-dataset. After finishing five training phases, we obtain the model CLIP$_5$. For comparison with CLIP$_{5}$, we retrain a CLIP$_{JT}$ as the upper bound of the CLIP$_{cl}$ based on the joint dataset of COCO and Flickr30K. The hyper-parameters for all training settings are kept the same, detailed settings of hyper-parameters can be seen in the Appendix\nzx{cite}.


%\textbf{Evaluation Metrics.} After completing the training on the t-th sub-dataset, we use the testsets of COCO(5K) and Flickr30k(1K) to test the multimodal retrieval performance of the CLIP$_t$ model, respectively.

\subsection{The Performance of Continual CLIP Training}
\label{explore_results}
\iffalse
First, we demonstrate the image-text retrieval performances of the CLIP$_0$ and CLIP$_{JT}$ on COCO (5K) and Flickr30K (1K) test sets in Table \ref{table:explore1}. 

\begin{table*}[!h]
%\vskip 0.15in
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{cl|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{Model}
& \multicolumn{6}{c}{Image-Text Retrieval} & \multicolumn{6}{c}{Text-Image Retrieval} \\
& & \multicolumn{3}{c}{Flickr30k} & \multicolumn{3}{c}{MSCOCO} & \multicolumn{3}{c}{Flickr30k} & \multicolumn{3}{c}{MSCOCO} \\
& & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
\midrule
COCO & CLIP$_{0}$ & \underline{16.9} & 37.0 & 46.2 & \underline{14.7} & 34.2 & 47.0 & \underline{12.0} & 30.0 & 41.0 & \underline{10.6} & 29.6 & 41.0 \\
COCO+Flickr30K & CLIP$_{JT}$ & \textbf{30.1} & 55.9 & 60.1 & \textbf{16.1} & 38.1 & 51.9 & \textbf{22.5} & 48.5 & 59.6 & \textbf{11.7} & 30.9 & 42.7 \\ %
\bottomrule
\end{tabular}
\caption{\textbf{The performance of CLIP in multimodal retrieval is affected by the training data domain.} Bold indicates the CLIP$_{JT}$'s R@1 results in COCO(5K) and Flickr30K(1K) test sets and underline indicates the CLIP$_0$'s R@1 results.}
\label{table:explore1}
\end{center}
\vspace{-1em}
\end{table*}

From the Table \ref{table:explore1}, we can find that the retrieval performance of CLIP$_{JT}$ on Flickr30k is significantly better than that of CLIP$_0$, which is not trained on Flickr30k. This phenomenon shows that the performance of the CLIP model is affected by the training data domain, which is consistent with the results of the paper \cite{radford2021learning}.
\fi
%首先我们展现了基于COCO数据集重训练的CLIP模型在COCO和Flickr30K数据集上的zero-shot图文检索能力。

We show the $R@1$ retrieval results of CLIP$_t$ $(0\leq t\leq 5)$ on the test set COCO(5K) and Flickr30K(1K) in Figure \ref{fig:base_retrival}. By comparing the performances of the CLIP$_0$ (initial phase) and CLIP$_{jt}$ on Flickr30K(1K), we can find that the retrieval performance of CLIP$_{jt}$ (red point) is significantly better than that of CLIP$_0$ (initial) which is not trained on Flickr30K. This phenomenon shows that \textbf{the performance of the CLIP model is affected by the training data domain}, which is consistent with the conclusion of the paper \cite{radford2021learning}. Besides this, it can be clearly seen that the multi-modal retrieval performance of the CLIP$_{ct}$ on the COCO(5K) declines continually with the rising of training phases. The final Image-Text R@1 result of CLIP$_5$ on COCO(5K) plummeted from the initial 14.7\% to 6.1\%, and the Text-Image results dropped from 10.6\% to 4.7\%. The gap with CLIP$_{jt}$ reached 10.0\% and 7.0\%, respectively. 
On the other hand, CLIP$_{ct}$ exhibits a slow and erratic increase in multi-modal retrieval $R@1$ results on the test set Flickr30K(1K). Although the results between CLIP$_{ct}$ and CLIP$_{jt}$ on the Image-Text $R@1$ has been narrowed from the original 13.2\% to 9.5\% while the Text-Image $R@1$ of CLIP$_{ct}$ has increased from 12.0\% to 16.1\%, the gap between CLIP$_5$ and CLIP$_{jt}$ is still great. %We name this phenomenon \textbf{Cognitive Disorder (CD)}.

%从图2中我们可以很明显的看出，随着连续预训练的持续进行CLIP模型在过去COCO数据域上的zero-shot 检索表现出现了持续的下降。虽然在当前训练域上的表现在上升，但最终模型的精度依旧与joint learning的结果差距明显。
\iffalse
\begin{figure}[h]
    \centering
	\subfigure{
	\centering
	\includegraphics[width=2.6in]{./figure/base_i2t_coco.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.6in]{./figure/base_t2i_coco.pdf}
	%\label{fig:tsne-c4il}
	}
	
	\subfigure{
	\centering
	\includegraphics[width=2.6in]{./figure/base_i2t_f30k.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.6in]{./figure/base_t2i_f30k.pdf}
	%\label{fig:tsne-c4il}
	}
	\caption{The multimodal retrieval $R@1$ results of CLIP$_t$ $(0\leq t\leq 5)$ on test sets COCO (5K) and Flickr30k (1K). The two sub-figures on the left show the Image-Text retrieval $R@1$ performance of CLIP$_t$ on the continual training phase $t$. The rights show the Text-Image $R@1$ results. The pentagon points (CLIP$_{jt}$) show the results of the CLIP under joint training, which is an upper bound for continual CLIP training (CLIP$_{ct}$).
	}
	\label{fig:base_retrival}
\end{figure}
\fi

\iffalse
\subsection{The Intra-Modal Rotation}
%在有监督的连续学习中，有一些工作从表征质量，概率分布等角度讨论了模型出现灾难性遗忘的原因。而在这里，我们将从一个全新的几何角度来讨论连续CLIP预训练中出现概念模糊的原因。希望这样的视角可以为连续学习社区提供新的启发。同时为探索导致模型在连续更新中表征质量下降的原因提供新的工具。
In supervised continual learning, there are some works that discussing the reasons for catastrophic forgetting of models in terms of representation quality\nzx{cite}, probability distribution\nzx{cite}, etc. In there, we will discuss the reasons for concept indistinct in continual CLIP pre-training from a geometrical perspective. 
\subsection{The inter-modal Deviation}
\subsection{Possibility of inter-modal Deviation}
\fi




























==> icml2023_hawaii_camera_ready__1_/content/5_reason.tex <==
\subsection{The reasons for catastrophic forgetting}
%在有监督的连续学习中，有一些工作从表征质量，概率分布等角度讨论了模型出现灾难性遗忘的原因。而在这里，我们将从一个全新的几何角度来讨论连续CLIP预训练中出现概念模糊的原因。希望这样的视角可以为连续学习社区提供新的启发。同时为探索导致模型在连续更新中表征质量下降的原因提供新的工具。
%In supervised continual learning, there are some works that discussing the reasons for catastrophic forgetting of models in terms of representation quality \cite{ni21revisit}, probability distribution \cite{ramasesh2020anatomy}, etc. In there, we will discuss the reasons for concept indistinct in continual CLIP pre-training from a geometrical perspective. 

%We can think of the D-dimensional output of the model as the representation vector of the sample in the model's representation space. The update of the model's parameters always leads to a change in the direction and length of the representation vector formed by it. Because of this, in continual training, we cannot judge what effect the length and direction changes of the vectors will have on the catastrophic forgetting of the model, respectively. 
In CLIP, the vision and language encoders normalize the final representation vector to a unit vector of length 1 using a dimension-based $L_2$ norm. 
\iffalse
\begin{equation}
|V^{D}| = |T^{D}| = 1
\end{equation}
where the $V^{D}$ and $T^{D}$ is the D-dimensional vision and language representation in CLIP. 
\fi
This design makes the representation space in vision and language encoders form a high-dimensional unit sphere, respectively. Therefore, we ignore the influence of the representation vectors' length and track their direction changes. We summarize these spatial variations as Spatial Disorder (SD), which can be divided into intra-modal rotation and inter-modal deviation.  
%我们可以将模型的D维输出视为样本在模型空间中的表征向量。而模型参数的更新则总是伴随着其表征向量方向和长度的双重变化。正因为如此，在连续训练过程中，我们无法控制变量的判断向量长度和方向对灾难性遗忘的影响。

%由于这样的模型设计使得无论模型如何更新，其输出的表征长度必为1。

\subsubsection{The Intra-modal Rotation}
\label{ImR}
Firstly, we analyze the directional changes of the representation vectors of model's vision and language extractors during continual CLIP training. Taking the visual representation space as an example, we use the visual encoder $E^V_{i}$ in CLIP$_{i}$ to extract the image representations of the test set COCO(5K) and obtain the vision representation vectors sets $V_{i}=\{V_i^0,...,V_i^N,...,V_i^{5K}\}$, where $i=0,...,5 $ stands for five different training phases. After that, we take the inner product of each pair of vectors $<V_i^a,V_i^b>$, where $a$ and $b$ are arbitrary indexes in each vector set $V_{i}$ and perform $arccos$ operation, the inverse trigonometric function of cosine, to obtain their \textbf{S}elf-\textbf{A}ngle relationship \textbf{M}atrix ($SAM_{i}$). The $SAM_i^{(a,b)} = arccos(<V_i^a,V_i^b>)$.
\iffalse
\begin{equation}
SAM_i^{(a,b)} = arccos(<V_i^a,V_i^b>)
\end{equation}
\fi
Any element $SAM_i^{(a,b)}$ in the $SAM_i$ matrix represents the included angle between the sample $a$ and $b$ in the vision encoder $E^V_i$. By counting the difference value $\theta_{SAM} = \angle (V_i^a,V_i^b) - \angle (V_{i+1}^a,V_{i+1}^b)$ between the corresponding elements in two continual $SAM$ matrix $SAM_i$ and $SAM_{i+1}$ as shown in Figure \ref{SAM_a}, we get the following included angle change distribution in Figure \ref{SAM_b}.

\begin{figure}[h]
%\vspace{-0.5em}
\subfigure[]{
\begin{minipage}[r]{0.5\linewidth}
\centering
\includegraphics[width = \linewidth]{./figure/SAM_2.pdf}
%\vspace{-1em}
\label{SAM_a}
\end{minipage}
}
\subfigure[]{
\begin{minipage}[l]{0.44\linewidth}
\centering
\includegraphics[width = \linewidth]{./figure/RAM_2.pdf}
%\caption{Example Image}
%\vspace{-1em}
\label{RAM_a}
\end{minipage}
}
%\vspace{-.5em}

\subfigure[]{
\setlength\tabcolsep{1pt}
\begin{minipage}[c]{1\linewidth}
%\tiny
\footnotesize
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 $\theta_{SAM} \in$ & $[0^{\circ}$, $5^{\circ}]$ & $(5^{\circ}$, $10^{\circ}]$ & $(10^{\circ}$, $15^{\circ}]$ & $(15^{\circ}$, $20^{\circ}] $ & $(20^{\circ}$, $180^{\circ}]$ \\
\midrule
$SAM_{0-1}$ &  54.23$\%$ & 31.64$\%$& 11.28$\%$ & 2.48$\%$ & 0.38$\%$ \\
$SAM_{1-2}$ &  61.18$\%$ & 30.21$\%$& 7.54$\%$ & 0.99$\%$ & 0.07$\%$ \\
$SAM_{2-3}$ &  61.44$\%$ & 30.00$\%$& 7.50$\%$ & 0.98$\%$ & 0.07$\%$ \\
$SAM_{3 - 4}$ &  55.33$\%$ & 31.75$\%$& 10.57$\%$ & 2.07$\%$ & 0.28$\%$ \\
$SAM_{4 - 5}$ &  50.51$\%$ & 32.14$\%$& 13.17$\%$ & 3.50$\%$ & 0.68$\%$ \\
$SAM_{0 - 5}$ &  42.94$\%$ & 31.12$\%$& 16.73$\%$ & 6.66$\%$ & 2.55$\%$ \\
\bottomrule
\end{tabular}
\label{SAM_b}
\end{minipage}
}
%\vspace{-1.5em}
\caption{The sub-figure on the (a) shows a schematic diagram of computing $\theta_{SAM}$. The sub-figure on the (b) shows a schematic diagram of computing $\theta_{RAM}$. The table on the bottom (c) shows the distribution of the change of the included angle between any two samples in different training phases' vision representation space. And $SAM_{i-j}$ = $|SAM_i - SAM_j|$.}
\label{SAM}
%\vspace{-0.5em}
\end{figure}

\iffalse
\begin{table*}[!h]
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 $\theta_{SAM} \in$ & $[0^{\circ}$, $5^{\circ}]$ & $(5^{\circ}$, $10^{\circ}]$ & $(10^{\circ}$, $15^{\circ}]$ & $(15^{\circ}$, $20^{\circ}] $ & $(20^{\circ}$, $180^{\circ}]$ \\
\midrule
$SAM_{0-1}$ &  54.23$\%$ & 31.64$\%$& 11.28$\%$ & 2.48$\%$ & 0.38$\%$ \\
$SAM_{1-2}$ &  61.18$\%$ & 30.21$\%$& 7.54$\%$ & 0.99$\%$ & 0.07$\%$ \\
$SAM_{2-3}$ &  61.44$\%$ & 30.00$\%$& 7.50$\%$ & 0.98$\%$ & 0.07$\%$ \\
$SAM_{3 - 4}$ &  55.33$\%$ & 31.75$\%$& 10.57$\%$ & 2.07$\%$ & 0.28$\%$ \\
$SAM_{4 - 5}$ &  50.51$\%$ & 32.14$\%$& 13.17$\%$ & 3.50$\%$ & 0.68$\%$ \\
$SAM_{0 - 5}$ &  42.94$\%$ & 31.12$\%$& 16.73$\%$ & 6.66$\%$ & 2.55$\%$ \\
\bottomrule
\end{tabular}
\caption{The table shows the angle change distribution of any two representation vectors in the visual extractor during continual CLIP training.}
\label{table:SAM}
\end{center}
\end{table*}
\fi

\iffalse
\begin{table*}[!h]
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 & $\theta \leq 5^{\circ}$ & $\theta \leq 10^{\circ}$ & $\theta \leq 15^{\circ}$ & $\theta \leq 20^{\circ}$ & $20^{\circ} \leq \theta $ \\
\midrule
$SAM_0 - SAM_1$ &  54.23$\%$ & 31.64$\%$& 11.28$\%$ & 2.48$\%$ & 0.38$\%$ \\
$SAM_1 - SAM_2$ &  71.54$\%$ & 24.89$\%$& 3.35$\%$ & 0.22$\%$ & 0.01$\%$ \\
$SAM_2 - SAM_3$ &  71.36$\%$ & 25.01$\%$& 3.40$\%$ & 0.22$\%$ & 0.01$\%$ \\
$SAM_3 - SAM_4$ &  67.30$\%$ & 27.27$\%$& 4.93$\%$ & 0.48$\%$ & 0.03$\%$ \\
$SAM_4 - SAM_5$ &  58.84$\%$ & 30.70$\%$& 8.77$\%$ & 1.50$\%$ & 0.20$\%$ \\
$SAM_0 - SAM_5$ &  55.39$\%$ & 31.60$\%$& 10.52$\%$ & 2.15$\%$ & 0.33$\%$ \\
\midrule
\end{tabular}
\caption{The table shows the angle difference distribution of any two representation vectors in the visual extractor during continual CLIP training.}
\label{table:SAM}
\end{center}
\end{table*}
\fi

From Figure \ref{SAM_b}, we can find that 80\% of the angle changes between any two vision representation vectors are between 0 and 10 degrees in continual training phases, while only 20\% are above 10 degrees. Moreover, less than 1\% of the angle changes are above 20 degrees. That angle changes between 15-20 degrees also only account for about 5\% of all image pairs. %Even comparing the angle changes of sample pair's between the initial model CLIP$_0$ and the final model CLIP$_5$, its distribution is also similar to others. 74\% of the sample pairs have a change in the included angle of less than 10 degrees. Only 2.55\% of the included angle changes are more than 20 degrees. 
Therefore, we conclude that \textbf{the topology of the visual representation of the CLIP$_{ct}$ changes slowly during the continual CLIP training.} In Appendix \ref{representation_quality}, we reached the same empirical conclusion by comparing the representation quality of vision encoders.% in different training phases.

\iffalse
We deduce that \textbf{the topology of the visual representation of the CLIP$_{cl}$ does not change significantly during the continual training}, and the angle structure between the sample pairs in the vision representation space before the update is preserved. This is very unusual to us, since the topology of the representation space is correlated with the quality of the model's representation. If the representational topology of the model does not change, then its representational quality should not change significantly either. To verify this, firstly, we freeze this six vision encoders' parameters. Then, using linear evaluation method \nzx{cite} commonly used in self-supervision to detect the classification accuracy of these six encoders on ImageNet\nzx{cite}. The final top-1 results are shown in the Figure.

\begin{figure}[h]
	\centering
	\includegraphics[height=1.8in]{./figure/top_1_imagenet.pdf}
	\caption{The linear evaluation results of this six vision encoders on ImageNet.}
	\label{process}
\end{figure}

The top-1 accuracy of the visual encoder $E_i^V$ in the CLIP$_{cl}$ on ImageNet did not show a significant decline and stabilized at 38\% $\pm$ 1, indicating that the representation quality of the visual encoder has not changed significantly during continual CLIP training. This also validates our inference that the topology of visual encoder in CLIP$_{cl}$ does not change significantly in continual training. 
\fi

In addition to discussing the change in the included angle between sample pairs in the visual representation space, by taking the inner product of the same sample's vision representation vector from different training phases' vision encoder $E_i^V$, we use the $arccos$ operation to compute the rotation angles $\theta_{RAM} = \angle (V_i^a,V_j^a)$ of each test sample $a$ in vision encoder $E_{i}^V$ and $E_{j}^V$ and get the \textbf{R}otation \textbf{A}ngle \textbf{M}atrix RAM$_{(i,j)}$. The $RAM_{(i,j)}^{a} = arccos(<V_i^a,V_j^a>)$. The schematic diagram can be seen in Figure \ref{RAM_a}. By counting the distribution of rotation angles, we get the following rotation angle distribution Table \ref{RAM}.


\iffalse
\begin{table*}[!h]
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 $\theta_{RAM} \in$ & $[0^{\circ}$, $15^{\circ}]$ & $(15^{\circ}$, $20^{\circ}]$ & $(20^{\circ}$, $25^{\circ}]$ & $(25^{\circ}$, $30^{\circ}] $ & $(30^{\circ}$, $180^{\circ}]$ \\
\midrule
$RAM_{(0,1)}$ &  0.00$\%$ & 0.20$\%$& 4.62$\%$ & 22.68$\%$ & 72.50$\%$ \\
$RAM_{(1,2)}$ &  0.00$\%$ & 0.40$\%$& 8.30$\%$ & 34.11$\%$ & 57.20$\%$ \\
$RAM_{(2,3)}$ &  0.00$\%$ & 0.30$\%$& 8.40$\%$ & 34.29$\%$ & 57.01$\%$ \\
$RAM_{(3,4)}$ &  0.00$\%$ & 0.00$\%$& 1.89$\%$ & 17.11$\%$ & 81.00$\%$ \\
$RAM_{(4,5)}$ &  0.00$\%$ & 0.00$\%$& 0.00$\%$ & 3.20$\%$ & 96.81$\%$ \\
$RAM_{(0,5)}$ &  0.00$\%$ & 0.00$\%$& 0.00$\%$ & 0.21$\%$ & 99.80$\%$ \\
\bottomrule
\end{tabular}
\caption{The table shows the rotation angle distribution of the same samples in the different vision representation spaces.}
\label{table:RAM}
\end{center}
\end{table*}
\fi

As shown in Table \ref{RAM}, we can find that the direction of the same sample in the visual representation space of different training phases has changed greatly. Only less than 0.4\% samples are rotated within 20 degrees in the continual CLIP training, while the samples rotated within 20-25 degrees are at most less than 9\%, and the samples of 25 degrees and above account for more than 90\%. We speculate that \textbf{the vision representation space of CLIP$_{ct}$ has undergone a large rotation around the high-dimensional sphere center during the continual training.} After analyzing the language representation space, we reach the same conclusion as the vision representation space. Detailed SAM and RAM of language encoders can be viewed in Appendix \ref{detail_language_encoder}.


\iffalse
The topological structure of the text representation space does not change significantly with the continual CLIP training. But the whole text representation space, like the visual representation space, has a large rotation around the center of the high-dimensional sphere in the continual training. The angle change distribution table \nzx{cite} and rotation angle distribution table \nzx{cite} are shown below. 

\begin{table*}[!h]
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
\subtable[The angle difference distribution in text representation space.]{
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 $\theta_{SAM} \in$ & $[0^{\circ}$, $5^{\circ}]$ & $(5^{\circ}$, $10^{\circ}]$ & $(10^{\circ}$, $15^{\circ}]$ & $(15^{\circ}$, $20^{\circ}] $ & $(20^{\circ}$, $180^{\circ}]$ \\
\midrule
$SAM_0 - SAM_1$ &  64.43$\%$ & 28.49$\%$& 6.23$\%$ & 0.78$\%$ & 0.07$\%$ \\
$SAM_1 - SAM_2$ &  71.54$\%$ & 24.89$\%$& 3.35$\%$ & 0.22$\%$ & 0.01$\%$ \\
$SAM_2 - SAM_3$ &  71.36$\%$ & 25.01$\%$& 3.40$\%$ & 0.22$\%$ & 0.01$\%$ \\
$SAM_3 - SAM_4$ &  67.30$\%$ & 27.27$\%$& 4.93$\%$ & 0.48$\%$ & 0.03$\%$ \\
$SAM_4 - SAM_5$ &  58.84$\%$ & 30.70$\%$& 8.77$\%$ & 1.50$\%$ & 0.20$\%$ \\
$SAM_0 - SAM_5$ &  55.39$\%$ & 31.60$\%$& 10.52$\%$ & 2.15$\%$ & 0.33$\%$ \\
\bottomrule
\end{tabular}
}

\subtable[The rotation angle distribution in text representation space.]{
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 $\theta_{RAM} \in$ & $[0^{\circ}$, $15^{\circ}]$ & $(15^{\circ}$, $20^{\circ}]$ & $(20^{\circ}$, $25^{\circ}]$ & $(25^{\circ}$, $30^{\circ}] $ & $(30^{\circ}$, $180^{\circ}]$ \\
\midrule
$RAM_{(0,1)}$ &  0.00$\%$ & 1.94$\%$& 28.38$\%$ & 45.88$\%$ & 23.80$\%$ \\
$RAM_{(1,2)}$ &  0.02$\%$ & 8.90$\%$& 47.76$\%$ & 34.94$\%$ & 8.38$\%$ \\
$RAM_{(2,3)}$ &  0.04$\%$ & 1.14$\%$& 49.86$\%$ & 31.18$\%$ & 7.52$\%$ \\
$RAM_{(3,4)}$ &  0.02$\%$ & 2.84$\%$& 33.70$\%$ & 43.76$\%$ & 19.68$\%$ \\
$RAM_{(4,5)}$ &  0.00$\%$ & 0.04$\%$& 3.28$\%$ & 27.66$\%$ & 69.02$\%$ \\
$RAM_{(0,5)}$ &  0.00$\%$ & 0.00$\%$& 0.00$\%$ & 1.12$\%$ & 98.88$\%$ \\
\bottomrule
\end{tabular}
}
\caption{\nzx{add captions}}
\label{table:text_analysis}
\end{center}
\end{table*}
\fi

According to our analysis of the geometric changes of the single-modal encoder's representation space during continual CLIP training, we conclude that: \textbf{During the continual CLIP training, the representation space in the CLIP$_{ct}$ is significantly rotated. The topology of the representation space is slightly rotated compared with the rotation of the whole representation space.} We name this phenomenon \textbf{Intra-modal Rotation}.

\begin{table}[h]
%\vspace{-0.5em}
%\vspace{-2em}
\iffalse
\subfigure[]{
\begin{minipage}[c]{1\linewidth}
\centering
\includegraphics[width = \linewidth]{./figure/RAM_2.pdf}
%\caption{Example Image}
\label{RAM_a}
\end{minipage}
}
\fi

\begin{minipage}[c]{1\linewidth}
\footnotesize
\setlength\tabcolsep{0.5pt}
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
 $\theta_{RAM} \in$ & $[0^{\circ}$, $15^{\circ}]$ & $(15^{\circ}$, $20^{\circ}]$ & $(20^{\circ}$, $25^{\circ}]$ & $(25^{\circ}$, $30^{\circ}] $ & $(30^{\circ}$, $180^{\circ}]$ \\
\midrule
$RAM_{(0,1)}$ &  0.00$\%$ & 0.20$\%$& 4.62$\%$ & 22.68$\%$ & 72.50$\%$ \\
$RAM_{(1,2)}$ &  0.00$\%$ & 0.40$\%$& 8.30$\%$ & 34.11$\%$ & 57.20$\%$ \\
$RAM_{(2,3)}$ &  0.00$\%$ & 0.30$\%$& 8.40$\%$ & 34.29$\%$ & 57.01$\%$ \\
$RAM_{(3,4)}$ &  0.00$\%$ & 0.00$\%$& 1.89$\%$ & 17.11$\%$ & 81.00$\%$ \\
$RAM_{(4,5)}$ &  0.00$\%$ & 0.00$\%$& 0.00$\%$ & 3.20$\%$ & 96.81$\%$ \\
$RAM_{(0,5)}$ &  0.00$\%$ & 0.00$\%$& 0.00$\%$ & 0.21$\%$ & 99.80$\%$ \\
\bottomrule
\end{tabular}
\end{minipage}
%\vspace{-.5em}
\caption{
The table on the bottom shows the rotation angle distribution of the same samples in different  training phases.}
\label{RAM}
\vspace{-1em}
\end{table}

%之后我们对每个向量集中的两两向量进行内积并求余弦之后获得他们各自的角度关系矩阵Self_Angle Matrix SAM_{i}。通过比较两个连续训练阶段的SAM矩阵中对应元素的差值，我们得到如下角度差值分布图。从图中我们可以发现在连续更新模型过程中视觉表征空间中的表征向量之间的角度差80%处在0-10度之间，而只有20%处在10度以上。同时，处于20度以上的只占了1%不到。15-20度之间的也只占了5%左右。即使是初始模型CLIP_0，其与最终模型CLIP_5之间的分布也如其他连续差值表现一样。这意味着向量V_i^a与向量V_i^b的夹角在连续更新过程中至少有85%的可能落在5度变化以内。这说明CLIP模型在连续的更新过程中其视觉表征的拓扑结构并没有出现明显的变化，原先样本间的角度差异被保留。这令我们感到非常惊讶，因为模型表征空间的拓扑结果与模型表征质量是完全相关的。如果模型的表征拓扑结构不变，则其表征质量也不应该有明显变化。为了验证这一点，我们将连续CLIP训练的得到的六个visionencoder参数全部冻结。使用自监督中常用的linear-evaluation的表征质量评估方式来检测这六个encoder在imagenet上的分类精度，最终的top-1结果如下表所示。可以发现随着连续训练的发生,CLIP_cl模型中的视觉encoder在imagenet上的top-1精度并没有出现明显的下滑。这也侧面验证了CLIP中的视觉编码器拓扑结构的确没有发生明显变化。

%之后，我们统计了不同训练阶段模型中的统一样本在视觉表征空间中的旋转角度。得到相对角度关系矩阵Relative_Angle_Matrix RAM_{i}. 通过统计相对角度分布，我们得到如下相对角度分布图。从图中我们可以发现同一样本在不同的训练阶段的视觉表征空间中所处的方位发生了巨大的变化。旋转20度以内的最多只占了4%，而旋转20-25度内的最多不到10%，而25度及以上的则占了90%以上。通过这两个现象，我们可以推测CLIP的视觉表征空间在连续更新过程中整个表征空间绕着球心进行了大幅度的旋转。对文字表征空间进行相同的分析之后，我们发现文字表征空间的变化也是如此。文字抽取器内部拓扑结构的变化相对整个空间结构的变化微乎其微。我们将这种现象称作模态内旋转。即CLIP模型在连续训练过程中其模态内的表征空间出现了大幅度的旋转，而其表征空间的拓扑结构则没有出现明显的变化。
\iffalse
\begin{figure}[h]
	\centering
	\includegraphics[height=1.8in]{./figure/RAM_difference_1.pdf}
	\caption{The comparison of the rotation distributions of the representation spaces of the vision and language extractors during continual CLIP training. CLIP$_{i-j}$ refers to the CLIP's continual training from training phase $i$ to $j$.}
	\label{RAM_difference}
\end{figure}
\fi
\begin{figure*}[h]
	\centering
	\includegraphics[height=2.2in]{./figure/RAM_difference_2.pdf}
    %\vspace{-.5em}
	\caption{The comparison of the rotation distributions of the vision encoder and langugae encoder during continual CLIP training. CLIP$_{i-j}$ refers to the CLIP's continual training from training phase $i$ to $j$. The values under the same color represent the proportion of test samples to total samples in each rotation angle interval of the same modality.}
	%\vspace{-0.5em}
	\label{RAM_difference}
%\vspace{-0.5em}
\end{figure*}
\subsubsection{The Inter-modal Deviation}
\label{ImD}
Although the topology of the single-modal representation space changes during continual training, this slight rotation should not be the main reason for the significant degradation of CLIP's multi-modal retrieval performance in continual training. To this end, we conduct a thought experiment: it is known that the representation spaces of vision and language encoders exhibit significant spatial rotations during continual training. Now we assume that the topology of the single-modal representation space is completely fixed during continual training. Therefore, if the CLIP$_{ct}$'s performance on multi-modal retrieval tasks does not degrade during continual training, \textbf{the rotations of the two encoders' representation spaces should be synchronized}. However, the fact is the \textbf{opposite}. So we think \textbf{there is a deviation between the rotation of the vision and language representation spaces}. Based on this suppose, we compare the rotation distributions of vision encoder (Table \ref{RAM}) and language encoder (Appendix \ref{detail_language_encoder}) and draw the rotation distribution comparison diagram (Figure \ref{RAM_difference}).
%The ordinate in the Figure \ref{RAM_difference} divides the rotation angle of the test samples before and after continual training into five angular intervals. 
The values under the same color represent the proportion of test samples to total samples in each rotation angle interval of the same modality. Comparing the difference in the distribution of rotation angles of the vision and language encoders, we can see that the space rotations of the two encoders are very different in the continual training. The rotation of language representation space is mostly concentrated between 20-30 degrees, while the vision's rotations are mostly between 30-180 degrees. This shows that the rotation of the representation space of the two modal extractors within CLIP$_{ct}$ is not synchronized during the continual training, which verifies our previous deduction: \textbf{The unsynchronized rotation of the vision and language representation spaces leads to representation space deviations between the CLIP's modal encoders (vision and language).} We name this phenomenon \textbf{Inter-modal Deviation}.
\iffalse
\begin{figure}[h]
	\centering
	\includegraphics[height=1.8in]{./figure/RAM_difference_2.pdf}
	\caption{The comparison of the rotation distributions of the representation spaces of the vision and language extractors during continual CLIP training. CLIP$_{i-j}$ refers to the CLIP's continual training from training phase $i$ to $j$.}
	\vspace{-0.5em}
	\label{RAM_difference}
\end{figure}
\fi
%单模态表征空间拓扑结构微小的变化会导致连续训练的CLIP模型出现如此明显的zero-shot检索表现下降吗？这不禁让我们提出疑问，是不是有其他原因在主导着模型的zero-shot表现？我们将目光重新放在了表征空间的旋转上。我们假设单模态表征空间的拓扑结构在连续CLIP训练中完全没有变化，而且连续CLIP预训练在zero-shot检索的表现不出现下降，那么成立的条件只有一个，就是单模态表征空间进行同步旋转或者不旋转！然而现在出现了zero-shot检索表现的下降，只能说明vision和text之间的表征空间的旋转并不是同步的。为此我们将图a和图b的旋转分布进行了对比，图z展现了两个模态表征空间的旋转差异。从...。这证实了我们的推论，即连续CLIP训练过程中，模型的两个模态各自出现的空间旋转并不是同步的。两个旋转之间存在明显差异，而这种差异导致过去相似度最高的图文样本在旋转中出现了Deviation。从而导致了模型在zero-shot检索结果上出现明显的下降。

%发现模态内的旋转让我们感到惊讶。一是CLIP在连续训练过程中，单模态的表征空间拓扑结构变化竟然不明显。这与传统的有监督连续学习大相径庭\cite{}。因为表征空间的拓扑结构变化总是对应模态表征质量的变化。
%\subsubsection{Intra-modal Rotation and Inter-modal Deviation lead to Spatial Disorder}
\begin{figure}[!h]
\subfigure[]{
\begin{minipage}[c]{1\linewidth}
\centering
\includegraphics[width = \linewidth]{./figure/relation_rot_4.pdf}
\end{minipage}
\label{relation_rot}
}
%\vspace{-1em}

\subfigure[]{
\begin{minipage}[c]{1\linewidth}
\centering
\includegraphics[width = \linewidth]{./figure/relation_dev_4.pdf}
\end{minipage}
\label{relation_dev}
}
%\vspace{-1em}
\caption{The Schematic illustration of spatial disorder caused by intra-modal rotation and inter-modal deviation. The $\alpha$ is vision representation and $\beta$ is language representation. The $a$,$b$ denote different image-text samples.
}
%\vspace{-1em}
\label{concept_indistinct}
\end{figure}
\begin{figure*}[!t]
	\centering
	\includegraphics[height=3.0in]{./figure/main_process_3.pdf}
	\caption{The Mod-X framework mainly consists of two sub-modules. Spatial Alignment helps the current model align the representation space of the old model based on current data. And Contrative helps the model fit the current training data domain. %The $S^{i,j}$ means cosine similarity score of the $i$'th sample's vision embedding and the $j$'th sample's text embedding.
    }
	\label{main_process}
%\vspace{-1.em}
\end{figure*}
\subsubsection{The Relationship between Spatial Disorder and Contrastive Matrix}
\label{relationshape_sd_cm}
How do spatial disorder cause the model to mis-align the old sample's vision and language representation? We show a schematic here to illustrate this. As shown in Figure \ref{concept_indistinct}, the $\alpha$ is vision representation and $\beta$ is language representation. The $a$,$b$ denote different image-text samples. 
For the convenience of illustration, we fix the vision vectors' relative location and rotate the language vectors to represent the unsynchronous rotation of the two modal spaces. 
When intra-modal rotation happens (Figure \ref{relation_rot}), $\beta_a$ in training phase $t+1$ is rotated to $\beta'_a$, the modal similarity between $a$ and $b$ shift from ($\beta_a^T \alpha_a > \beta_a^T \alpha_b$) to ($\beta{'}_a^T\alpha_a < \beta{'}_a^T\alpha_b$), which break the alignment of the current model to old sample $a$. The superscript $T$ is a transpose operation that is often used for matrix multiplication.
%When training in phase $t$, affected by training data domain $t$, the CLIP$_t$ aligned sample $a$ but ignored sample $b$ where the ($<\beta_b,\alpha_b>\quad<\quad<\beta_b,\alpha_a>$). However, due to the topological structure of the encoder space is only slightly changed, 
When inter-modal deviation happens (Figure \ref{relation_dev}), %the model updating it's parameters in training phase $t+1$ to align the sample $b$, which exist in training data domain $t+1$, 
the relative rotation of the representation space breaks the original modal alignment of the sample $a$, which makes the ($\beta_a^T\alpha_b > \beta_a^T\alpha_a$). 
From the perspective of the contrastive matrix, the element $M_{i,j}$ in the $i$,$j$ position of the contrastive matrix $M$ represents the similarity score of the $i$'th sample vision embedding and the $j$'th sample text embedding. Since the length of the representation vector is \textbf{1}, the similarity score $M_{i,j}$ also refers to the angle between the $i$'th sample vision embedding and the $j$'th sample text embedding. When the angle becomes larger due to spatial disorder, its similarity score within the model becomes smaller, which affects the multi-modal retrieval ability of the model. Because of this, the performance of CLIP$_{ct}$ drops significantly during continual training. Detailed mathematical derivations can be found in Appendix \ref{theoretical}. The value of the diagonal elements in the contrast matrix $M$ represents the angle between different modals of the same sample. The value of the off-diagonal elements represents the angle between the different modals of different samples in the CLIP's representation space. %When the include angle between Through our exploration (in section \ref{explore}), the Intra-modal Rotation and the Inter-modal Deviation affect these angles or similarity scores. 
From an overall perspective, \textbf{the similarity distribution of the contrastive matrix $M$ is equivalent to the structure of the representation space of the model.} 
%To this end, we abstract this problem and give the theoretical conditions that the inter-modal deviation leads to the wrong retrieval results of the model. That is, when the relative rotation between the vision and language representation space is greater than 90 degrees, the retrieval result of the model must be wrong. The theoretical analysis can be seen in Appendix \ref{theoretical}.
%在这里，我们讨论模态间偏离如何导致模型的概念模糊。正如


==> icml2023_hawaii_camera_ready__1_/content/6_method.tex <==
\section{Alleviating Spatial Disorder}
\label{method}
\subsection{General continual CLIP training Setting}
Suppose we have used training dataset $D_0$ got a pre-trained model CLIP$_0$. And there is another vision-language dataset $D$. We split $D$ into $N$ sub-datasets $\{D_1, ..., D_N\}$, randomly and evenly, to simulate a stream of data and $D_t= \{(v_t^0,l_t^0),...,(v_t^{n},l_t^{n})\}$ denotes the training data in the training phase $t$, where $t \in \{1,2,...,N\}$. Then, we train the model CLIP$_0$ using this sub-datasets sequentially. The enocded $l_2$ normalized embeddings of vision and text is $V_t^i=E_V^t(v_t^i)$ and $L_t^i=E_L^t(l_t^i)$. When the model CLIP$_t$ is trained during the training phase $t$ using training data $D_t$, the previous sub-datasets $\{D_0, D_1, ..., D_{t-1}\}$ are no longer available. The joint training represents that training a CLIP$_{jt}$ from scratch using all data $D_{jt} = D_0 \cup D$.

\subsection{Mod-X: Maintain off-diagonal information-matrix}
To alleviate spatial disorder of the CLIP$_{ct}$ model during continual training. We propose a simple but effective new training framework: Maintain off-diagonal information-matrix (Mod-X). It boots the current CLIP model to retain the spatial alignment to past samples by distilling the contrastive matrix's off-diagonal information which is constructed by the model before and after continual training based on the current training data. The entire training framework is shown in Figure \ref{main_process}, where the $S^{i,j}$ means cosine similarity score of the $i$'th sample's vision embedding and the $j$'th sample's text embedding. The Contrastive module in Figure \ref{main_process} is a traditional InfoNCE loss \cite{baevski2020wav2vec} , which inherits from CLIP \cite{radford2021learning}. In the following, we mainly introduce our Spatial Alignment module. 

\iffalse
\begin{figure*}[h]
	\centering
	\includegraphics[height=2.8in]{./figure/main_process_8.pdf}
	\caption{The Mod-X framework mainly consists of two subsections. Cognition Align helps the current model align the cognition of the old model based on current data. And Contrative helps the model fit the current training data domain. The $S^{i,j}$ means cosine similarity score of the $i$'th sample vision embedding and the $j$'th sample text embedding.}
	\label{main_process}
\end{figure*}
\fi

%为了缓解CLIP模型在连续训练过程中的概念模糊。我们提出了一个新的模块：Maintain off-diagonal information-matrix(Mod-X).他通过蒸馏连续训练前后模型对当前数据的相似度矩阵中的非对角线信息来保存当前训练模型对之前样本模态间概念的对齐。从而缓解连续训练过程中的概念模糊。整个连续训练框架如下图所示。
\iffalse
\subsection{Contrastive Module}
CLIP$_t$ trains its own vision and language encoders $E_V^t$ and $E_L^t$ by minimizing the contrastive loss $L_{InfoNCE} = L_V + L_L$ , where $L_V$ is the loss for aligning vision to language and $L_L$ is the loss for aligning language to vision. Take the $L_V$ for example:

\begin{equation}
L_V = - \frac{1}{n}\sum^n_{i=1}\sum_{j=1}^nI_{ij}log[Sim(v^i,l^j;\tau)]
\end{equation}
where the $Sim(v^i,l^j;\tau)$ function is:
\begin{equation}
Sim(v^i,l^j;\tau) = \frac{exp(s(v^i,l^j / \tau))}{\sum_{k=1}^N exp(s(v^i,l^k / \tau))}
\end{equation}

The $s(v^i,l^k) = (v^i)^Tl^k$ is the cosine similarity function and $\tau$ is a temperature parameter can be set or learned. By pulling together the visual and textual representations of the same sample and pushing away the similarity between different sample, the CLIP learns how to distinguish and identify different samples through the similarity of multimodal.
\fi

\subsection{Spatial Alignment}
The diagonal elements in CLIP's contrastive matrix represent the similarity of the visual and language information of the current sample. The off-diagonal elements represent the similarity between the vision and language representation of the current sample and other samples. As mentioned in Section \ref{relationshape_sd_cm}, the distribution of the elements in the contrastive matrix represents the spatial distribution of representations between modalities of the model.
%The distribution of off-diagonal elements in the contrastive matrix represents the current model's cognition about the current training objects. 
Therefore, we feel out the old model's representation space through the old model's contrastive matrix on the current training data. Then, selectively distill the old model's spatial distribution while training the current model. We construct contrastive matrix $M_{t-1}$ and $M_t$ using the last and current model CLIP$_{t-1}$ and CLIP$_{t}$ based on current sub-dataset $D_t$.
\begin{gather}
    M_{t-1}^{i,j} = CLIP_{t-1}(D_t) = s(E_V^{t-1}(v_{t}^i),E_L^{t-1}(l_{t}^j))  \\
    M_{t}^{i,j} = CLIP_{t}(D_t) = s(E_V^{t}(v_{t}^i),E_L^{t}(l_{t}^j)) 
\end{gather}

Where the $s(a,b) = a^Tb$ is the cosine similarity function. However, the last model's representation space for current data is not totally correct. For those misunderstood sample information (diagonal elements are not the largest in the current retrieval), we use the corresponding similarity information of the current model to replace them, thereby removing their influence during continual distillation. %We called this \textbf{Screening}.
\begin{equation}
M_{t-1}^{(i,:)} = M_t^{(i,:)} ; \quad if \quad max(M^i_{t-1}) \neq i
\end{equation}
After that, we align the information matrix $M_{t-1}$ and $M_{t}$ using Kullback-Leibler Divergence \cite{csiszar1975divergence}.
\begin{equation}
L_{KL}^t(M_t,M_{t-1}) = -\sum M_{t-1} ln(\frac{M_t}{M_{t-1}})
\end{equation}

The final training loss can be written as $L_{Mod-X}$, and $\alpha$ is a hyper-parameter.
\begin{equation}
L_{Mod-X}^t = L_{InfoNCE}^t + \alpha L_{KL}^t
\end{equation}

%CLIP的训练基于模型对样本的视觉和文字模态信息对之间的相似性。其对比矩阵的对角线元素代表了模型对当前样本的视觉与文字模态的相似性评分。而非对角线元素则表示了当前样本的视觉模态与其他样本的文字模态之间的相似度。反之亦然。也就是说对比矩阵中的非对角线元素的分布代表了当前模型对事物的概念图。也是当前模型内视觉与文字标准模态的匹配图。因此，蒸馏CLIP模型训练前后对当前数据的非对角线信息矩阵就是在蒸馏模型内部模态间的匹配关系。然而过去的模型对当前样本的理解并不一定是完全正确的。也就是对角线值并不一定全是当前行中最大的。对于这些样本，我们将其替换成当前模型所构建对比矩阵的对应行信息。从而忽略蒸馏过程中的错误概念。










==> icml2023_hawaii_camera_ready__1_/content/7_experiment.tex <==
\section{Experiments}
\label{experiments}
\subsection{Training Datasets}
In the experiments, we use three image-text datasets varying in scale and scope to simulate continual CLIP training.
\textbf{MS COCO Captions} \cite{lin2014microsoft}: MS COCO Captions (COCO) is a widely used image caption dataset. It contains 80K training images, 30K validation images, and 5K testing images (COCO(5K)). Each image has 5 human-evaluated captions.
\textbf{Flickr30K} \cite{young2014image}: Flickr30K(F30K) contains 30K training images and 1K test samples (Flickr30K(1K)) collected from Flickr, together with 5 reference sentences provided by human annotators. \textbf{SBU-1M} \cite{ordonez2011im2text}: The SBU-1M collects 1M images from Flickr with associated visually relevant captions which representing a wider variety of content styles. After downloading and preprocessing, we utilized about 0.8M image-text pairs in our experiments. 

\subsection{Experiments Setting}
We apply our Mod-X framework to two experiment settings to illustrate that Mod-X helps the model not only better fits the newly trained data domain but also maintains the multimodal cognitive ability of the old data domain during the continual large-scale training.
\textbf{Experiment A:} The Experiment A follows the setup of the exploratory experiments, pre-training the CLIP$_0$ model using the COCO dataset. And then splitting Flickr30K dataset randomly and evenly into five sub-datasets and sequentially training them to update CLIP$_0$ continually.
\textbf{Experiment B:} Unlike Experiment A, which looks like fine-tuning, we try to simulate continual large-scale training in Experiment B. We train a CLIP from scratch using the joint data of COCO and Flickr30K (COCO+F30K) as the initial model CLIP$_0$ and continually train eight sub-datasets divided from the SBU-1M dataset, randomly and uniformly. Each sub-dataset contains 100K unique samples, an equal scale to the initial pre-training dataset (COCO+F30K). This experiment verifies that our framework can iterate under continual large-scale training and maintain or even improve the model’s cognition of past entities.
\textbf{Evaluation Details:} We use the test sets COCO(5K) and Flickr30K(1K) to evaluate the performance of model in continual training. And all the results in the tables and figures are the average of 3 runs with different seeds. Experiment details have been shown in Appendix \ref{Experiment_Setting}.

\iffalse
\subsection{Experiments Details}
\textbf{Training Details} We use ResNet50 \cite{he2016deep} as the vision encoder in CLIP, while the language encoder is a transformer-based architecture which follows modification proposed in CLIP \cite{OpenAi}. The input images are resized to 224 × 224 and the input texts are tokenized by WordPiece with a maximum length of 77. We utilize AdamW \cite{loshchilov2017decoupled} optimizer and a cosine annealing learning rate schedule with warmup which is consistent with \cite{OpenAi}. All of the experiments are conducted on 8 NVIDIA V100 GPUS. Details regarding hyper-parameter values for different experiments are provided in the Appendix \nzx{cite}.

\textbf{Evaluation Details.} We use the test sets of COCO(5K) and Flickr30K to evaluate the zero-shot image-text retrieval performance of CLIP model. 
\fi


\subsection{Performance of Mod-X in the Experiment A}
\label{experiment_A}
\iffalse
In figure \ref{fig:modx_f30k} , we show the effect of our framework Mod-X with (CLIP$_{Mod-X}$) or without (CLIP$_{w/o}$) Screening in continual CLIP training in Experiment A.
\begin{figure}[!h]
    \centering
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_i2t_coco.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_t2i_coco.pdf}
	%\label{fig:tsne-c4il}
	}
	
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_i2t_f30k.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_t2i_f30k.pdf}
	%\label{fig:tsne-c4il}
	}
	\caption{\nzx{need caption}
	}
	\label{fig:modx_f30k}
\end{figure}

From the results of zero-shot retrieval at each training phase, we can find that our framework, Mod-X, still has a good performance to the past pre-training dataset COCO during the continual training on the Flickr30K dataset. At each training phases, the zero-shot results of CLIP$_{Mod-X}$ on COCO(5K) testset does not show a significant drop, and the gap with the initial accuracy remained at $\pm 1$. In addition to this, by comparing the zero-shot retriveal results of the CLIP$_{cl}$ and CLIP$_{Mod-X}$ on the current training data domain (Flickr30K), it can be found that the CLIP$_{Mod-X}$ using the off-diagonal information before and after the model update is also significantly better than CLIP$_{cl}$ in continual fitting the current data domain. 
\fi

The Experiment A focuses on verifying that Mod-X can not only fit new data domains but also maintain a cognition of past data domains. This table shows the final multimodal retrieval performance of the different training strategies on COCO(5K) and Flickr30K(1K). The CLIP$_0$ is the initial pre-trained model based on the COCO dataset. The CLIP$_{ct}$ means training CLIP continually without any other operation. The CLIP$_{EWC}$ means using the EWC method \cite{kirkpatrick2017overcoming}, which is a typical regularization strategy in continual supervised learning. The CLIP$_{Mod-X}$ is the proposed Mod-X, and the CLIP$_{JT}$ is the joint training model using the joint datasets (COCO+F30K), which is an upper bound for continual CLIP training in Experiment A. The detailed performance of the different models at each training phase is shown in Appendix \ref{detailed_A}.

\begin{table*}[!h]
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
& & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
& & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
\multirow{4}{*}{COCO} & CLIP$_{0}$ & \overline{16.9} & 37.0 & 46.2 & \overline{14.7} & 34.2 & 47.0 & \overline{12.0} & 30.0 & 41.0 & \overline{10.6} & 29.6 & 41.0  \\
 & CLIP$_{ct}$ & 20.6 & 42.8 & 56.4 & 6.2 & 17.8 & 26.1 & 16.1 & 38.5 & 50.4 & 4.7 & 14.3 & 21.8 \\
 & CLIP$_{EWC}$ & 22.2 & 43.1 & 57.0 & 6.1 & 17.2 & 26.5 & 17.0 & 39.1 & 51.2 & 4.5 & 13.9 & 22.0 \\
 %& CLIP$_{w/o}$ & 24.9 & 50.4 & 60.3 & 7.6 & 21.4 & 30.9 & 19.4 & 43.2 & 54.6 & 6.0 & 17.4 & 25.7 \\
 & CLIP$_{Mod-X}$ & \textbf{27.9} & \textbf{53.4} & \textbf{64.4} & \textbf{14.5} & \textbf{34.0} & \textbf{46.1} & \textbf{20.2} & \textbf{45.0} & \textbf{57.2} & \textbf{10.1} & \textbf{26.4} & \textbf{37.4} \\
\midrule
COCO+F30K & CLIP$_{jt}$ & \underline{30.1} & 55.9 & 60.1 & \underline{16.1} & 38.1 & 51.9 & \underline{22.5} & 48.5 & 59.6 & \underline{11.7} & 30.9 & 42.7 \\ %
\bottomrule
\end{tabular}
\caption{The final multimodal retrieval performance of the different continual CLIP training strategies in the Experiment A.}
\label{table:modx_f30k}
\end{center}
\vspace{-0.5em}
\end{table*}
%The underlined values represent the upper bound for continual training of the CLIP. And the bold ones are the results of our framework Mod-X. 
From the results in the Table \ref{table:modx_f30k}, it is clear that our method CLIP$_{Mod-X}$
%it can be found that the final performance of our method far exceeds the results of CLIP$_{cl}$.
maintains its multimodal retrieval results on COCO(5K) after completing continual training on Flickr30K. The gap between CLIP$_0$ and CLIP$_{Mod-X}$ is just 0.2\% points in image-text retrieval and 0.5\% points in text-image retrieval on COCO(5K). At the same time, the retrieval results of the CLIP$_{Mod-X}$ on the test set Flickr30K(1K) are also affected by the training domain and have a significant increase. The $R@1$ performance of the CLIP$_{Mod-X}$ in image-text retrieval rise from 16.9\% (in CLIP$_0$) to 27.9\%. And the $R@1$ results in text-image retrieval increase from 12.0\% (in CLIP$_0$) to 20.2\%. The performance gap between CLIP$_{Mod-X}$ and CLIP$_{jt}$ on the Flickr30K is only at most 2.3\% points. Conversely, due to the model's cognitive disorder in continual training, the performance of CLIP$_{ct}$ on COCO(5K) drops significantly. In addition, although the performance of CLIP$_{ct}$ on Flickr30K(1K) has improved, it is still far from the upper bound CLIP$_{jt}$. The EWC, as a typical regularization strategy in continual learning, selectively updates the model by evaluating the importance of each parameter of the model. From the above experimental results, although CLIP$_{EWC}$ improves the accuracy of continual CLIP training on Flickr30K(1K), it does not preserve the model's understanding in past samples (COCO(5K)). According to the above comparisons, we can conclude that our Mod-X framework can not only maintain the cognitive ability on past samples during continual CLIP learning but also improve the model's fitting ability to the current training data domain.


%outperforms CLIP$_{cl}$ 7.3 and 8.3 points on Image-Text retrieval results. In the Text-Image retrieval results, it also exceeds 4.1 and 5.4 points. Compared with the upper bound CLIP$_{JT}$, the gap is only 2.3 points at most (the R@1 result in Text-Image Retrival on Flickr30K). The low performance of traditional regularization methods EWC also shows that multi-modal continual training is more complex than single-modal supervised training. 

%Beside this, we compare the performance of Mod-X with CLIP$_{Mod-X}$ and without CLIP$_{w/o}$ Screening during continual training in Experiment A. We can see that the multimodal retrieval performance of Mod-X without the Screening CLIP$_{w/o}$ in the COCO data domain is only 1 point higher than that of CLIP$_{cl}$, and the gap with CLIP$_{Mod-X}$ is obvious. Moreover, the results of CLIP$_{w/o}$ is also lower than CLIP$_{Mod-X}$ on the current Flickr30K data damain (3 points in image-text $R@1$ and 0.8 points in text-image $R@1$ on Flickr30K). All of this shows that Screening plays an important role in Mod-X. Aligning this misunderstanding of the old model with the concept of new objects will affect the parameter update of the entire CLIP model in the continual training. 

%从每个阶段zero-shot retrieval的结果中我们可以看出我们的新框架ModX在F30K数据集上进行连续更新的过程中其对过去的预训练数据集COCO的拟合能力依旧很好。其zero-shot retrieval的表现没有出现明显的下降（正负1）。这说明我们的方法的确帮助模型缓解了对过去样本的概念模糊。除此以往，通过比较模型在当前训练数据集（Flickr30K）上的zero-shot retriveal表现可以发现，我们的方法在拟合当前数据时由于对非对角线信息的保存，使得最终的拟合效果也明显优于continual training。下表展示了CLIP_Mod-X模型在连续更新之后的最终表现。
\iffalse
\subsection{The importance of Screening}
To illustrate the importance of Screening, we compare the performance of Mod-X with and without Screening during continual training in Experiment A. The results of CLIP$_{w/o}$ can be seen in figure \ref{table:modx_f30k}. We can see that the zero-shot retrieval performance of Mod-X without the Screening CLIP$_{w/o}$ drops significantly. At the same time, the performance of the CLIP$_{w/o}$ in the current data domain (Flisckr30K) also fluctuates significantly during the continual training compared to CLIP$_{Mod-X}$. Comparing the final retrieval results of the three training strategies in Table \ref{table:modx_f30k}, it can be find that the performance of the CLIP without Screening CLIP$_{w/o}$ in the past data domain is only 1 point higher than that of CLIP$_{cl}$, and the gap with CLIP$_{Mod-X}$ is obvious. Moreover, the results of CLIP$_{w/o}$ is also lower than CLIP$_{Mod-X}$ on the current data damain (3 points in image-text $R@1$ and 0.8 points in text-image $R@1$ on Flickr30K). All of this shows that Screening plays an important role in Mod-X. Aligning this misunderstanding of the old model with the concept of new objects can affect the parameter update of the entire model in the continual training.
\fi

\subsection{Performance of Mod-X in the Experiment B}
\label{experiment_B}
%In the Experiments B,  we use SBU1M dataset to simulate large-scale continual CLIP training. The difference from the Experiment A is that we use COCO+F30K as the pre-training data for the initial pre-trained model CLIP$_0$. Joint Datasets are the union of COCO, F30K and SBU1M. And the number of training phases increased from 5 to 8. The amount of training data in each training phase reaches 100K which is approximately equal with pre-trained datasets COCO and F30K.
Unlike Experiment A, which looks like fine-tuning, Experiment B focuses on verifying that our framework Mod-X can maintain or even improve the model’s understanding of past entities when iterating under continual large-scale training. Table \ref{table:modx_sbu1m} shows the final multimodal retrieval performance of the different continual CLIP training strategies in Experiment B. The detailed $R@1$ results in each training phase can be seen in Appendix \ref{detailed_B}.

\begin{table*}[!h]
\vspace{-0.5em}
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
& & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
& & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
\multirow{4}{*}{COCO+F30K} & CLIP$_{0}$ & \overline{33.0} & 56.5 & 67.3 & \overline{17.7} & 40.7 & 52.9 & \overline{23.4} & 48.2 & 59.1 & \overline{12.9} & 32.8 & 44.9  \\
 & CLIP$_{ct}$ & 5.4 & 16.0 & 23.3 & 3.0 & 9.0 & 14.0 & 3.6 & 12.0 & 18.6 & 2.3 & 7.3 & 11.4 \\
 & CLIP$_{EWC}$ & 6.1 & 18.2 & 33.5 & 3.1 & 11.7 & 18.2 & 3.3 & 10.4 & 16.2 & 2.1 & 5.4 & 10.0 \\
 %& CLIP$_{w/o}$ & 24.9 & 50.4 & 60.3 & 7.6 & 21.4 & 30.9 & 19.4 & 43.2 & 54.6 & 6.0 & 17.4 & 25.7 \\
 & CLIP$_{Mod-X}$ & \textbf{37.3} & \textbf{62.6} & \textbf{72.1} & \textbf{19.5} & \textbf{42.8} & \textbf{55.7} & \textbf{26.0} & \textbf{51.9} & \textbf{62.6} & \textbf{13.4} & \textbf{33.6} & \textbf{45.3} \\
\midrule
Joint Datasets & CLIP$_{jt}$ & \underline{39.3} & 71.5 & 81.1 & \underline{25.1} & 51.6 & 64.3 & \underline{27.8} & 54.9 & 66.5 & \underline{15.9} & 38.6 & 51.3 \\ %
\bottomrule
\end{tabular}
\caption{The final multimoal retrieval performance of the different continual CLIP training strategies in the Experiment B.}
\label{table:modx_sbu1m}
\end{center}
\vspace{-0.5em}
\end{table*}

Compared to the initial pre-trained model CLIP$_0$, our CLIP$_{Mod-X}$ not only does not show a significantly drop such as CLIP$_{ct}$ in multimodal retrieval performance on COCO(5K) and Flickr30K(1K) but it also shows a slight improvement after continual training in SBU-1M. The image-text $R@1$ results on Flickr30K(1K) increase from 33.0\% to 37.3\% and the accuracy on COCO improved to 19.5\% from 17.7\%. The performance of text-image $R@1$ is the same as that of image-text. The accuracy increase from 23.4\% to 26.0\% on Flickr30K(1K) and 12.9\% to 13.4\% on COCO(5K). The gap between continual CLIP training and joint training has been somewhat narrowed. Conversely, the ability of cognitive alignment in CLIP$_{ct}$ and CLIP$_{EWC}$ are lost in the large-scale data. This results in verifying that our framework Mod-X can iterate under continual large-scale training and can maintain or even improve the model’s cognitive ability of past entity concepts.






==> icml2023_hawaii_camera_ready__1_/content/7_experiment_change.tex <==
\section{Experiments}
\label{experiments}
\subsection{Datasets}
In the experiments, we use three different training datasets varying in scope and domain to evaluate the effectiveness of our Mod-X framework. \textbf{MS COCO Captions} \cite{lin2014microsoft}: MS COCO Captions (COCO) is a widely used image caption dataset. It contains 80K training images, 30K validation images, and 5K testing images (COCO(5K)). \textbf{Flickr30K} \cite{young2014image}: Flickr30K contains 30K training images and 1K test samples (Flickr30K(1K)) collected from Flickr, together with 5 reference sentences provided by human annotators. \textbf{ECommerce-T2I} \cite{M6-T} is a text-to-image e-commerce dataset that contains 90k training images and 5k testing images set (EC(5K)). Each image corresponds to a text description, and the description for each sample in the training and test sets does not repeat. Many detailed training settings and experiments (CC12M) can be viewed in Appendix \ref{Appendix_to_experiments}. 


%results of other datasets(SBU-1M and CC12M) and all of training settings can be viewed in appendix \nzx{cite}. 
%\textbf{CC12M} training dataset \cite{changpinyo2021conceptual} collects about 12M images and their raw descriptions harvested from the alt-text HTML attribute associated with the webscraped images, therefore representing a wider variety of content styles. Due to unavailable URLs, we utilize about 10M examples from this dataset. The experimental results of more datasets and settings can be viewed in appendix \nzx{cite}
\iffalse
\subsection{Experiments Setting}
We apply our Mod-X framework to two experiment settings to illustrate that Mod-X helps the model not only better fits the newly trained data domain but also maintains the multimodal representation alignment of the old data domain during the continual large-scale training.
\textbf{Experiment A:} The Experiment A follows the setup of the exploratory experiments, pre-training the CLIP$_0$ model using the COCO dataset. And then splitting Flickr30K dataset randomly and evenly into five sub-datasets and sequentially training them to update CLIP$_0$ continually.
\textbf{Experiment B:} Unlike Experiment A, which looks like training in similarity data domain, we try to simulate continual training in a different domain in Experiment B. We splitting ECommerce-T2I training dataset randomly and evenly into five sub-datasets and sequentially training them to update pre-trained model CLIP$_0$ continually.
%We train a CLIP from scratch using the joint data of COCO and Flickr30K (COCO+F30K) as the initial model CLIP$_0$ and continually train eight sub-datasets divided from the SBU-1M dataset, randomly and uniformly. Each sub-dataset contains 100K unique samples, an equal scale to the initial pre-training dataset (COCO+F30K). This experiment verifies that our framework can iterate under continual large-scale training and maintain or even improve the model’s cognition of past entities.
\textbf{Evaluation Details:} We use the test sets COCO(5K) and Flickr30K(1K) to evaluate the performance of model in continual training. And all the results in the tables and figures are the average of 3 runs with different seeds. Experiment details have been shown in Appendix \ref{Experiment_Setting}.
\fi

\iffalse
\subsection{Experiments Details}
\textbf{Training Details} We use ResNet50 \cite{he2016deep} as the vision encoder in CLIP, while the language encoder is a transformer-based architecture which follows modification proposed in CLIP \cite{OpenAi}. The input images are resized to 224 × 224 and the input texts are tokenized by WordPiece with a maximum length of 77. We utilize AdamW \cite{loshchilov2017decoupled} optimizer and a cosine annealing learning rate schedule with warmup which is consistent with \cite{OpenAi}. All of the experiments are conducted on 8 NVIDIA V100 GPUS. Details regarding hyper-parameter values for different experiments are provided in the Appendix \nzx{cite}.

\textbf{Evaluation Details.} We use the test sets of COCO(5K) and Flickr30K to evaluate the zero-shot image-text retrieval performance of CLIP model. 
\fi

\begin{figure}[!h]
    %\vspace{-1.em}
    \centering
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/A_i2t_coco_cam_2.pdf}
	%\label{fig:tsne-icarl}
	}
    %\vspace{-1.4em}
    
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/A_t2i_coco_cam_2.pdf}
	%\label{fig:tsne-c4il}
	}
    %\vspace{-1.4em}
	
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/A_i2t_f30k_cam_2.pdf}
	%\label{fig:tsne-icarl}
	}
    %\vspace{-1.4em}
    
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/A_t2i_f30k_cam_2.pdf}
	%\label{fig:tsne-c4il}
	}
    \vspace{-2em}
	\caption{The multi-modal retrieval $R@1$ results of the different training strategies on COCO(5K) and Flickr30K(1K). The first two sub-figures show the retrieval $R@1$ performance on previous COCO dataset. The last two sub-figures show the $R@1$ results on current training domain Flickr30K.}%The pentagon points (CLIP$_{jt}$) show the results of the CLIP under joint training, which is an upper bound for CLIP training.}
	\label{fig:modx_f30k_official}
\vspace{-1.em}
\end{figure}
\subsection{The performance in Exploratory Experiments}
\label{experiment_A}
\iffalse
In figure \ref{fig:modx_f30k} , we show the effect of our framework Mod-X with (CLIP$_{Mod-X}$) or without (CLIP$_{w/o}$) Screening in continual CLIP training in Experiment A.
\begin{figure}[!h]
    \centering
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_i2t_coco.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_t2i_coco.pdf}
	%\label{fig:tsne-c4il}
	}
	
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_i2t_f30k.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=2.65in]{./figure/A_t2i_f30k.pdf}
	%\label{fig:tsne-c4il}
	}
	\caption{\nzx{need caption}
	}
	\label{fig:modx_f30k}
\end{figure}
From the results of zero-shot retrieval at each training phase, we can find that our framework, Mod-X, still has a good performance to the past pre-training dataset COCO during the continual training on the Flickr30K dataset. At each training phases, the zero-shot results of CLIP$_{Mod-X}$ on COCO(5K) testset does not show a significant drop, and the gap with the initial accuracy remained at $\pm 1$. In addition to this, by comparing the zero-shot retriveal results of the CLIP$_{cl}$ and CLIP$_{Mod-X}$ on the current training data domain (Flickr30K), it can be found that the CLIP$_{Mod-X}$ using the off-diagonal information before and after the model update is also significantly better than CLIP$_{cl}$ in continual fitting the current data domain. 
\fi
\begin{figure*}[!t]
    \centering
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/EC_I2T_EC_2.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/EC_T2I_EC_2.pdf}
	%\label{fig:tsne-c4il}
	}
    %\vspace{-1.em}
 
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/EC_I2T_coco_2.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/EC_T2I_coco_2.pdf}
	%\label{fig:tsne-c4il}
	}
    %\vspace{-1.em}
	
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/EC_I2T_f30k_2.pdf}
	%\label{fig:tsne-icarl}
	}
	\subfigure{
	\centering
	\includegraphics[width=3.2in]{./figure/EC_T2I_f30k_2.pdf}
	%\label{fig:tsne-c4il}
	}
    %\vspace{-1.em}
	\caption{The retrieval $R@1$ performance of different training strategies in each training phase on EC(5K), COCO(5K) and Flickr30K(1K). The CLIP$_{ft}$ is the fine-tuning results of CLIP$_{initial}$ on the full ECommerce-T2I dataset as an upper bound on CLIP$_{ct}$.}
	\label{fig:modx_ec_offifial}
    \vspace{-.5em}
\end{figure*}
Firstly, we follow the setup of the exploratory experiments described in Section \ref{explore_results}, comparing the results of our Mod-X framework with CLIP$_{ct}$, CLIP$_{EWC}$ and CLIP$_{jt}$ in the Flickr30K dataset. The CLIP$_{ct}$ means training CLIP continually without any other operation. The CLIP$_{jt}$ is training CLIP model in the joint dataset of COCO and Flickr30K, which is an upper bound for continual CLIP training. Since label information is not used in CLIP training, recent supervised continual training methods like iCaRL \cite{rebuffi2017icarl}, PodNet \cite{douillard2020podnet}, and Dyn \cite{yan2021dynamically} cannot be reproduced in such experimental settings. We compared our Mod-X with the typical continual learning strategy such as DER \cite{buzzega2020dark} (CLIP$_{DER}$), EWC \cite{kirkpatrick2017overcoming} (CLIP$_{EWC}$) and LWF \cite{li2017learning} (CLIP$_{LWF}$). Notably, to make LWF and DER work properly within the CLIP framework, we reproduced them using contrastive loss replaced their cross-entropy loss. The replay buffer size of DER is set to 3000. Figure \ref{fig:modx_f30k_official} shows the effect of our framework Mod-X (CLIP$_{Mod-X}$) and the performance of other training strategies at each training phase. At each training phase, the $R@1$ results of CLIP$_{Mod-X}$ on COCO(5K) did not show a significant drop, and the gap with the initial accuracy (\textit{Initial}) remained at $\pm 1\%$. Additionally, by comparing the retrieval performance of the CLIP$_{ct}$ and CLIP$_{Mod-X}$ on the current training data domain (Flickr30K), it can be found that the CLIP$_{Mod-X}$ is also significantly better than CLIP$_{ct}$ in continual fitting the current data domain. The low performance of CLIP$_{EWC}$ and CLIP$_{LWF}$ also shows that continual multi-modal training is more complex than single-modal supervised training. Due to the use of old training samples in memory buffer, the performance of DER is slightly better than LWF. However, its performance is still far from that of Mod-X. 
\begin{table}[!t]
\begin{minipage}[c]{1\linewidth}
\footnotesize
\setlength\tabcolsep{0.5pt}
\begin{tabular}{cc c}
\toprule
 Methods & COCO(I2T/T2I) & Flickr30K (I2T/T2I) \\
\midrule
$CLIP_{jt}$ &  16.1 / 11.7 & 	30.1 / 22.5 \\
$CLIP_{Mod-X}$ with 5000 &  15.3 / 11.0 & 29.1 / 21.7 \\
$CLIP_{Mod-X}$ with 3000 &  15.0 / 10.8 & 28.5 / 21.0 \\
$CLIP_{Mod-X}$ &  14.5 / 10.1	& 27.9 / 20.2 \\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-.5em}
\caption{
The table show the R@1 performance of the Mod-X framework in the final phase with a buffer size of 3000 or 5000. Since memory buffer strategy stores the model's knowledge from the input, it remains effective in the Mod-X framework which does not limit the input form.}
\label{memory_bank}
\vspace{-1em}
\end{table}
In Table \ref{memory_bank}, we presents the R@1 performance of the Mod-X framework in the final phase with a memory buffer size of 3000 or 5000. Before training on the Flickr30K, we randomly saved 1000 training samples from the COCO dataset into the memory buffer. Afterward, based on the size of the buffer, an equal number of current training samples were randomly selected and stored in the memory buffer after each continual training phase which is similar to previous works \cite{rebuffi2017icarl,buzzega2020dark,douillard2020podnet}. Since memory buffer strategy stores the model's knowledge from the input, it remains effective in the Mod-X framework which does not limit the input form. We can see from the results that as the number of old samples used increases, the performance of the Mod-X becomes closer to joint training. 

Beside of this, in order to show the performance of our Mod-X in high semantics correlations data sets, we adopt an approximate strategy to simulate class incremental setting in Flickr30K. Considering that the image labels are not available in Flickr30K, we used a pre-trained Imagenet1K model to automatically label the Flickr30K training data and divided it into 5 subsets, with each subset containing 200 classes. The R@1 results in the final phase have shown in Table \ref{cls_modx}, where the "cls" means "class incremental setting". From the results, it seems that continuous training with class incremental setting did not have a heavy impact on the effectiveness of the Mod-X. 
\begin{table}[!t]
\begin{minipage}[c]{1\linewidth}
\footnotesize
\setlength\tabcolsep{0.5pt}
\begin{tabular}{cc c}
\toprule
 Methods & COCO(I2T/T2I) & Flickr30K (I2T/T2I) \\
\midrule
$CLIP_{Mod-X}$ &  14.5 / 10.1	& 27.9 / 20.2 \\
$CLIP_{Mod-X}$ with cls &  13.8/9.8	& 27.4/19.7 \\
$CLIP_{ct}$ &  	6.2/4.7	& 20.6/16.1 \\
$CLIP_{ct}$ with cls &  6.3/4.7 & 18.1/15.7 \\
\bottomrule
\end{tabular}
\end{minipage}
%\vspace{-.5em}
\caption{
The table show the R@1 performance of the Mod-X framework in a class incremental setting. The results demonstrate that continuous training with class incremental setting did not have a heavy impact on the effectiveness of the Mod-X.}
\label{cls_modx}
\vspace{-1em}
\end{table}
In Appendix \ref{relationship_cm_ims_modx}, we show the spatial alignment in CLIP$_{Mod-X}$ and CLIP$_{ct}$, which demonstrates that the Mod-X framework can alleviate the spatial disorder well during continual CLIP training. 

\iffalse
\begin{table*}[!h]
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
& & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
& & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
\multirow{4}{*}{COCO} & CLIP$_{0}$ & \overline{16.9} & 37.0 & 46.2 & \overline{14.7} & 34.2 & 47.0 & \overline{12.0} & 30.0 & 41.0 & \overline{10.6} & 29.6 & 41.0  \\
 & CLIP$_{ct}$ & 20.6 & 42.8 & 56.4 & 6.2 & 17.8 & 26.1 & 16.1 & 38.5 & 50.4 & 4.7 & 14.3 & 21.8 \\
 & CLIP$_{EWC}$ & 22.2 & 43.1 & 57.0 & 6.1 & 17.2 & 26.5 & 17.0 & 39.1 & 51.2 & 4.5 & 13.9 & 22.0 \\
 %& CLIP$_{w/o}$ & 24.9 & 50.4 & 60.3 & 7.6 & 21.4 & 30.9 & 19.4 & 43.2 & 54.6 & 6.0 & 17.4 & 25.7 \\
 & CLIP$_{Mod-X}$ & \textbf{27.9} & \textbf{53.4} & \textbf{64.4} & \textbf{14.5} & \textbf{34.0} & \textbf{46.1} & \textbf{20.2} & \textbf{45.0} & \textbf{57.2} & \textbf{10.1} & \textbf{26.4} & \textbf{37.4} \\
\midrule
COCO+F30K & CLIP$_{jt}$ & \underline{30.1} & 55.9 & 60.1 & \underline{16.1} & 38.1 & 51.9 & \underline{22.5} & 48.5 & 59.6 & \underline{11.7} & 30.9 & 42.7 \\ %
\bottomrule
\end{tabular}
\caption{The final multimodal retrieval performance of the different continual CLIP training strategies in the Experiment A.}
\label{table:modx_f30k}
\end{center}
\vspace{-0.5em}
\end{table*}
%The underlined values represent the upper bound for continual training of the CLIP. And the bold ones are the results of our framework Mod-X. 
From the results in the Table \ref{table:modx_f30k}, it is clear that our method CLIP$_{Mod-X}$
%it can be found that the final performance of our method far exceeds the results of CLIP$_{cl}$.
maintains its multimodal retrieval results on COCO(5K) after completing continual training on Flickr30K. The gap between CLIP$_0$ and CLIP$_{Mod-X}$ is just 0.2\% points in image-text retrieval and 0.5\% points in text-image retrieval on COCO(5K). At the same time, the retrieval results of the CLIP$_{Mod-X}$ on the test set Flickr30K(1K) are also affected by the training domain and have a significant increase. The $R@1$ performance of the CLIP$_{Mod-X}$ in image-text retrieval rise from 16.9\% (in CLIP$_0$) to 27.9\%. And the $R@1$ results in text-image retrieval increase from 12.0\% (in CLIP$_0$) to 20.2\%. The performance gap between CLIP$_{Mod-X}$ and CLIP$_{jt}$ on the Flickr30K is only at most 2.3\% points. Conversely, due to the model's cognitive disorder in continual training, the performance of CLIP$_{ct}$ on COCO(5K) drops significantly. In addition, although the performance of CLIP$_{ct}$ on Flickr30K(1K) has improved, it is still far from the upper bound CLIP$_{jt}$. The EWC, as a typical regularization strategy in continual learning, selectively updates the model by evaluating the importance of each parameter of the model. From the above experimental results, although CLIP$_{EWC}$ improves the accuracy of continual CLIP training on Flickr30K(1K), it does not preserve the model's understanding in past samples (COCO(5K)). According to the above comparisons, we can conclude that our Mod-X framework can not only maintain the cognitive ability on past samples during continual CLIP learning but also improve the model's fitting ability to the current training data domain.
\fi

%outperforms CLIP$_{cl}$ 7.3 and 8.3 points on Image-Text retrieval results. In the Text-Image retrieval results, it also exceeds 4.1 and 5.4 points. Compared with the upper bound CLIP$_{JT}$, the gap is only 2.3 points at most (the R@1 result in Text-Image Retrival on Flickr30K). The low performance of traditional regularization methods EWC also shows that multi-modal continual training is more complex than single-modal supervised training. 

%Beside this, we compare the performance of Mod-X with CLIP$_{Mod-X}$ and without CLIP$_{w/o}$ Screening during continual training in Experiment A. We can see that the multimodal retrieval performance of Mod-X without the Screening CLIP$_{w/o}$ in the COCO data domain is only 1 point higher than that of CLIP$_{cl}$, and the gap with CLIP$_{Mod-X}$ is obvious. Moreover, the results of CLIP$_{w/o}$ is also lower than CLIP$_{Mod-X}$ on the current Flickr30K data damain (3 points in image-text $R@1$ and 0.8 points in text-image $R@1$ on Flickr30K). All of this shows that Screening plays an important role in Mod-X. Aligning this misunderstanding of the old model with the concept of new objects will affect the parameter update of the entire CLIP model in the continual training. 

%从每个阶段zero-shot retrieval的结果中我们可以看出我们的新框架ModX在F30K数据集上进行连续更新的过程中其对过去的预训练数据集COCO的拟合能力依旧很好。其zero-shot retrieval的表现没有出现明显的下降（正负1）。这说明我们的方法的确帮助模型缓解了对过去样本的概念模糊。除此以往，通过比较模型在当前训练数据集（Flickr30K）上的zero-shot retriveal表现可以发现，我们的方法在拟合当前数据时由于对非对角线信息的保存，使得最终的拟合效果也明显优于continual training。下表展示了CLIP_Mod-X模型在连续更新之后的最终表现。
\iffalse
\subsection{The importance of Screening}
To illustrate the importance of Screening, we compare the performance of Mod-X with and without Screening during continual training in Experiment A. The results of CLIP$_{w/o}$ can be seen in figure \ref{table:modx_f30k}. We can see that the zero-shot retrieval performance of Mod-X without the Screening CLIP$_{w/o}$ drops significantly. At the same time, the performance of the CLIP$_{w/o}$ in the current data domain (Flisckr30K) also fluctuates significantly during the continual training compared to CLIP$_{Mod-X}$. Comparing the final retrieval results of the three training strategies in Table \ref{table:modx_f30k}, it can be find that the performance of the CLIP without Screening CLIP$_{w/o}$ in the past data domain is only 1 point higher than that of CLIP$_{cl}$, and the gap with CLIP$_{Mod-X}$ is obvious. Moreover, the results of CLIP$_{w/o}$ is also lower than CLIP$_{Mod-X}$ on the current data damain (3 points in image-text $R@1$ and 0.8 points in text-image $R@1$ on Flickr30K). All of this shows that Screening plays an important role in Mod-X. Aligning this misunderstanding of the old model with the concept of new objects can affect the parameter update of the entire model in the continual training.
\fi

\iffalse
\subsection{The performance of Mod-X when continual training the OpenAI's CLIP on COCO and Flickr30K}
We set the CLIP$_{vit32}$ as the initial model in the continuous training process and divide the joint-dataset (COCO and Flickr30K) into five sub-datasets uniformly and randomly to simulate streaming data. Because the pre-training datasets of CLIP$_{vit32}$ are not available, we train CLIP$_{vit32}$ on the joint-dataset to get the model CLIP$_{ft}$ as an upper bound for the performance of continual training. We apply our framework Mod-X in this setting and compare the final multimodal retrieval results with CLIP$_{ct}$, which is just continual training without any other operations, in Table \ref{table:modx_vit}.

\begin{table*}[h]
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
 & \multicolumn{3}{c}{Flickr30k(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30k(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
 & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
  CLIP$_{vit32}$ & \overline{77.7} & 94.5 & 98.3 & \overline{50.1} & 74.6 & 83.0 & \overline{58.9} & 83.5 & 90.1 & \overline{30.2} & 55.6 & 66.7  \\
  CLIP$_{ct}$ & 85.6 & 96.3 & 98.8 & 59.7 & 83.2 & 90.2 & 71.2 & 91.5 & 94.9 & 43.5 & 70.9 & 80.6 \\
  CLIP$_{Mod-X}$ & \textbf{86.1} & \textbf{97.0} & \textbf{99.1} & \textbf{62.1} & \textbf{85.6} & \textbf{91.7} & \textbf{72.4} & \textbf{92.5} & \textbf{96.2} & \textbf{46.2} & \textbf{72.9} & \textbf{82.0} \\
\midrule
  CLIP$_{ft}$ & \underline{86.3} & 97.2 & 99.1 & \underline{63.6} & 86.4 & 92.3 & \underline{72.7} & 92.6 & 96.3 & \underline{46.3} & 73.1 & 82.3 \\ %
\bottomrule
\end{tabular}
\caption{The final multimoal retrieval performance of the CLIP$_{ct}$, CLIP$_{Mod-X}$ and CLIP$_{ft}$ based on OpenAI's CLIP$_{vit32}$ with VIT-32/B vision encoder.}
\label{table:modx_vit}
\end{center}
\end{table*}

The performance of our framework Mod-X is still better than CLIP$_{ct}$ on all of the evaluation settings. Comparing the $R@1$ results on the test set Flickr30K(1K), we can find that CLIP$_{Mod-X}$ not only surpasses the initial results (CLIP$_{vit32}$) but also 1.3\% points and 2.2\% points higher than CLIP$_{ct}$. The results on COCO(5K) also illustrate that our framework not only resists the cognitive disorder of the model but also fits the new data domain better than CLIP$_{ct}$. The $R@1$ results of CLIP$_{Mod-X}$ on COCO(5K) surpasses the CLIP$_{ct}$ by 2.4\% and 2.7\% points, respectively.
\fi

\subsection{The performance on special domain dataset ECommerce-T2I}
\label{Experiments_ECommerce-T2I}
To illustrate that the Mod-X framework is not only applicable to similar data domains, in this section, we compare the performance of different continual training frameworks on a specific e-commerce dataset ECommerce-T2I. We set the CLIP$_{vit32}$ with ViT-Base/32 vision encoder as the initial model, pre-trained using large-scale open-world datasets in \cite{OpenAi}. To simulate streaming data, we are dividing the entire ECommerce-T2I into five sub-datasets uniformly and randomly. Since the entire CLIP$_{vit32}$ pre-training dataset is not available, we use the fine-tuning results of CLIP$_{vit32}$ on the entire ECommerce-T2I dataset (CLIP$_{ft}$) as an upper bound on CLIP$_{ct}$.


%CLIP$_{Mod-X}$ with CLIP$_{ct}$, CLIP$_{EWC}$ and CLIP$_{ft}$ for continual training 

\iffalse
\begin{table*}[h]
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
 \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
 & \multicolumn{2}{c}{Flickr30k(1K)} & \multicolumn{2}{c}{COCO(5K)} & \multicolumn{2}{c}{EC(5K)} & \multicolumn{2}{c}{Flickr30k(1K)} & \multicolumn{2}{c}{COCO(5K)} & \multicolumn{2}{c}{EC(5K)}\\
 & $R@1$ & $R@5$ & $R@1$ & $R@5$ & $R@1$ & $R@5$ & $R@1$ & $R@5$ & $R@1$ & $R@5$ & $R@1$ & $R@5$ \\
\midrule
  CLIP$_{vit32}$ & 77.7 & 94.5 & 50.1 & 74.6 & 11.3 & 27.6 & 58.9 & 83.5 & 30.2 & 55.6 & 10.1 & 25.5  \\
  CLIP$_{ct}$ & 63.4 & 87.2 & 36.8 & 61.5 & 16.6 & 40.7 & 44.4 & 71.0 & 20.6 & 42.6 & 15.8 & 40.5 \\
  CLIP$_{Mod-X}$ & \textbf{73.1} & \textbf{92.1} & \textbf{47.1} & \textbf{70.5} & \textbf{20.1} & \textbf{44.8} & \textbf{55.6} & \textbf{79.9} & \textbf{27.9} & \textbf{51.0} & \textbf{20.0} & \textbf{44.8} \\
\midrule
  CLIP$_{ft}$ & 64.5 & 88.6 & 39.8 & 64.8 & 23.5 & 50.8 & 46.9 & 73.1 & 22.2 & 44.5 & 23.5 & 50.6 \\ %
\bottomrule
\end{tabular}
\caption{The final multimoal retrieval performance of the CLIP$_{ct}$, CLIP$_{Mod-X}$ and CLIP$_{ft}$ based on OpenAI's CLIP$_{vit32}$ on specific e-commerce data domain (ECommerce-T2I).}
\label{modx_vit_ec}
\end{center}
\end{table*}
\fi

The multi-modal retrieval $R@1$ results of CLIP$_{Mod-X}$, CLIP$_{ct}$, CLIP$_{EWC}$ and CLIP$_{ft}$ in each training phase are shown in Figure \ref{fig:modx_ec_offifial}. Comparing the $R@1$ performance of the CLIP$_{jt}$ and CLIP$_{ct}$ on the EC(5K) test set, it's clear that the training of the CLIP model is affected by the training data domain: The final $R@1$ results of CLIP$_{jt}$ on EC(5K) is 8.8\% (Image-Text) and 9.9\% points (Text-Image) higher than CLIP$_{ct}$. However, the retrieval results of CLIP$_{jt}$ on COCO(5K) and Flickr30K(1K) have dropped by more than 10\% points (comparing with CLIP$_{vit32}$ (\textit{Initial})) on average, which means that the performance of fine-tuning (one phase continual training) CLIP is also affected by the data domain. This is also verified by observations that the $R@1$ performance of CLIP$_{ct}$ performs lower than CLIP$_{jt}$. On the contrary, the CLIP$_{Mod-X}$ obtained after continual training by the Mod-X framework only has a tie drop of 3.3\% points in the $R@1$ retrieval results on COCO(5K) and Flickr30K(1K). What's more, the performance of the CLIP$_{Mod-X}$ on EC(5K) outperformed CLIP$_{ct}$ by 3.5\% (Image-Text R@1) and 4.2\% points (Text-Image R@1), respectively. The overall $R@1$ trend of CLIP$_{EWC}$ is similar to that of CLIP$_{ct}$ but is more unstable than CLIP$_{ct}$. All of this shows that Mod-X framework not only preserves the inter-modal spatial structure of old samples during the continual training but also improves the fitting ability of the CLIP in the current training data domain. 

\iffalse
\subsection{Performance of Mod-X in the Experiment B}
\label{experiment_B}
%In the Experiments B,  we use SBU1M dataset to simulate large-scale continual CLIP training. The difference from the Experiment A is that we use COCO+F30K as the pre-training data for the initial pre-trained model CLIP$_0$. Joint Datasets are the union of COCO, F30K and SBU1M. And the number of training phases increased from 5 to 8. The amount of training data in each training phase reaches 100K which is approximately equal with pre-trained datasets COCO and F30K.
Unlike Experiment A, which looks like fine-tuning, Experiment B focuses on verifying that our framework Mod-X can maintain or even improve the model’s understanding of past entities when iterating under continual large-scale training. Table \ref{table:modx_sbu1m} shows the final multimodal retrieval performance of the different continual CLIP training strategies in Experiment B. The detailed $R@1$ results in each training phase can be seen in Appendix \ref{detailed_B}.

\begin{table*}[!h]
\vspace{-0.5em}
%\vspace{-1em}
\small
\begin{center}
\setlength\tabcolsep{1.8pt}
%\resizebox{\textwidth}{mm}
\begin{tabular}{c|l|ccc|ccc|ccc|ccc}
\toprule
\multirow{3}{*}{\shortstack[c]{Pretraining\\ Dataset}} & \multirow{3}{*}{\shortstack[c]{Model}} & \multicolumn{6}{c}{Image-Text Retrieval(\%)} & \multicolumn{6}{c}{Text-Image Retrieval(\%)} \\
& & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} & \multicolumn{3}{c}{Flickr30K(1K)} & \multicolumn{3}{c}{COCO(5K)} \\
& & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ & $R@1$ & $R@5$ & $R@10$ \\
\midrule
\multirow{4}{*}{COCO+F30K} & CLIP$_{0}$ & \overline{33.0} & 56.5 & 67.3 & \overline{17.7} & 40.7 & 52.9 & \overline{23.4} & 48.2 & 59.1 & \overline{12.9} & 32.8 & 44.9  \\
 & CLIP$_{ct}$ & 5.4 & 16.0 & 23.3 & 3.0 & 9.0 & 14.0 & 3.6 & 12.0 & 18.6 & 2.3 & 7.3 & 11.4 \\
 & CLIP$_{EWC}$ & 6.1 & 18.2 & 33.5 & 3.1 & 11.7 & 18.2 & 3.3 & 10.4 & 16.2 & 2.1 & 5.4 & 10.0 \\
 %& CLIP$_{w/o}$ & 24.9 & 50.4 & 60.3 & 7.6 & 21.4 & 30.9 & 19.4 & 43.2 & 54.6 & 6.0 & 17.4 & 25.7 \\
 & CLIP$_{Mod-X}$ & \textbf{37.3} & \textbf{62.6} & \textbf{72.1} & \textbf{19.5} & \textbf{42.8} & \textbf{55.7} & \textbf{26.0} & \textbf{51.9} & \textbf{62.6} & \textbf{13.4} & \textbf{33.6} & \textbf{45.3} \\
\midrule
Joint Datasets & CLIP$_{jt}$ & \underline{39.3} & 71.5 & 81.1 & \underline{25.1} & 51.6 & 64.3 & \underline{27.8} & 54.9 & 66.5 & \underline{15.9} & 38.6 & 51.3 \\ %
\bottomrule
\end{tabular}
\caption{The final multimoal retrieval performance of the different continual CLIP training strategies in the Experiment B.}
\label{table:modx_sbu1m}
\end{center}
\vspace{-0.5em}
\end{table*}

Compared to the initial pre-trained model CLIP$_0$, our CLIP$_{Mod-X}$ not only does not show a significantly drop such as CLIP$_{ct}$ in multimodal retrieval performance on COCO(5K) and Flickr30K(1K) but it also shows a slight improvement after continual training in SBU-1M. The image-text $R@1$ results on Flickr30K(1K) increase from 33.0\% to 37.3\% and the accuracy on COCO improved to 19.5\% from 17.7\%. The performance of text-image $R@1$ is the same as that of image-text. The accuracy increase from 23.4\% to 26.0\% on Flickr30K(1K) and 12.9\% to 13.4\% on COCO(5K). The gap between continual CLIP training and joint training has been somewhat narrowed. Conversely, the ability of cognitive alignment in CLIP$_{ct}$ and CLIP$_{EWC}$ are lost in the large-scale data. This results in verifying that our framework Mod-X can iterate under continual large-scale training and can maintain or even improve the model’s cognitive ability of past entity concepts.
\fi

\iffalse
\subsection{Other Results }
Beside of this two experiments, in appendix \ref{}, we show the Mod-X's performance in continual training the CLIP model from scratch on large-scale dataset CC12M. The multi-modal zero-shot retrieval performance and zero-shot classification results also demonstrate that our Mod-X framework still performs better than single continual training in large-scale pre-training.
\fi










==> icml2023_hawaii_camera_ready__1_/content/8_conclusion.tex <==
\section{Conclusion}
This paper discusses the feasibility of continuously training the CLIP model through streaming data. Then, by tracking the directional changes of the representation vectors in the continuously updated CLIP model, we explore and summarize these spatial variations as Spatial Disorder (SD), which can be divided into Intra-modal Rotation and Inter-modal Deviation. Moreover, we demonstrate how intra-modal rotation and inter-modal deviation lead to a performance decline for CLIP on cross-modal retrieval tasks in both empirically and theoretically. To alleviate the spatial disorder, we propose a simple yet effective continual learning framework Mod-X: \textbf{M}aintain \textbf{o}ff-\textbf{d}iagonal information-matri\textbf{X}. The experiments (in Section \ref{method}, \ref{experiments} and Appendix \ref{Appendix_to_experiments}) on commonly used datasets with different scales and scopes have illustrated the effectiveness of our method.

%The results in experiments (section \ref{experiment_A} and section \ref{Experiments_ECommerce-T2I}) demonstrate the effectiveness of our framework. More experimental results and details can be seen in the Appendix.

%Mod-X not only better fits the newly trained data domain (Section \ref{experiment_A}), but also maintains the multimodal concept alignment of the old data domain during the continual large-scale training (Section \ref{experiment_B}).

%Through selectively aligning the off-diagonal information distribution of the contrastive matrix, the Mod-X not only better fits the newly trained data domain (Section \ref{experiment_A}), but also maintains the multimodal concept alignment of the old data domain during the continual large-scale training (Section \ref{experiment_B}).


%By selectively distilling the off-diagonal information distributions in the contrastive matrix before and after training, Mod-X better fits the current training data domain while aligning the concept understanding of objects between the past CLIP and present CLIP. The performance in two experiments A and B \ref{experiments} with different scale and scope datasets shows that our Mod-X framework can effectively alleviate concept indistinct which makes training CLIP model continuously through streaming data feasibility.

%In this paper, we explore the feasibility of training CLIP model continuously through streaming data and name the decline in multimodal retrieval results for CLIP during continual training as Concept Indistinct. Then, by analyzing the changes in the spatial topology of the CLIP representation, we illustrate two reasons for the concept indistinct of the CLIP during continual training. The first is Intra-modal Rotation. It refers to the fact that during the continual CLIP training, the representation space of vision and text encoders rotates greatly around the center of the high-dimensional sphere, while the topology of the encoders does not change much relative to the rotation of the representation space. The second is Inter-modal Deviation. It refers to the fact that the representation spaces of the two encoders are rotated out of synchronization during continual training, resulting in deviations in the similarity between modalities. What's more, we mathematically give the conditions under which the inter-modal deviation causes concept indistinct in the continual CLIP training. To alleviate the concept indistinct of the continual CLIP training, we propose a new continual learning framework Mod-X: \textbf{M}aintain \textbf{o}ff-\textbf{d}iagonal information-matri\textbf{X}. By selectively distilling the off-diagonal information distributions in the contrastive matrix before and after training, Mod-X better fits the current training data domain while aligning the concept understanding of objects between the last CLIP and present CLIP.

%\textbf{Limitation:} Although our method performs well on both large and small scale datasets, our experimental datasets are all open-world. We do not discuss the effect in the case of a specific data domain (such as commodity, food, etc.). For the case of large deviations in the data domain, we conjecture that adding some past samples to the current training may be helpful in alleviating the conceptual ambiguity of the model.














